PrivacyProxy: Leveraging Crowdsourcing and In Situ Traffic Analysis to Detect and Mitigate Information Leakage

Many smartphone apps transmit personally identifiable information (PII), often without the users knowledge. To address this issue, we present PrivacyProxy, a system that monitors outbound network traffic and generates app-specific signatures to represent sensitive data being shared. PrivacyProxy uses a crowd-based approach to detect likely PII in an adaptive and scalable manner by anonymously combining signatures from different users of the same app. Furthermore, we do not observe users network traffic and instead rely on hashed signatures. We present the design and implementation of PrivacyProxy and evaluate it with a lab study, a field deployment, a user survey, and a comparison against prior work. Our field study shows PrivacyProxy can automatically detect PII with an F1 score of 0.885. PrivacyProxy also achieves an F1 score of 0.759 in our controlled experiment for the 500 most popular apps. The F1 score also improves to 0.866 with additional training data for 40 apps that initially had the most false positives. We also show performance overhead of using PrivacyProxy is between 8.6% to 14.2%, slightly more than using a standard unmodified VPN, and most users report no perceptible impact on battery life or the network.

==> 05_evaluation_original.tex <==
\section{Evaluation}
\label{sec:Evaluation}

\begin{table*}
\caption{Summary Table showing detection efficiency in the controlled experiment and in the field deployment. Row 2 and row 3 show the performance of \PP for the \totalAppsForMoreTraining apps which had maximum number of false positives after 1 and 7 rounds of training runs.} 
% \JH{Why is this caption text in all caps?}
% This is the IEEE format: Captions in small caps above the table and captions in small letters below figures
\label{tab:precision}

\small
\centering
\begin{tabular}{|l*{5}{|c}|r|}
	\hline
    \textbf{Scenario} & \textbf{TP} & \textbf{FP} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\
 	\hline 
    \hline
	\parbox[c]{3cm}{\vspace{1mm} Controlled Experiment\\ \vspace{1mm}} & \TPControlled & \FPControlled & \FNControlled & \PrecisionControlled & \RecallControlled & \FScoreControlled \\ \hline
    \hline
    \parbox[c]{3cm}{\vspace{1mm} Additional Training\\ Experiment (Round 1) \vspace{1mm}} & \TPAdditionalTrainingStart & \FPAdditionalTrainingStart & \FNAdditionalTrainingStart & \PrecisionAdditionalTrainingStart & \RecallAdditionalTrainingStart & \FScoreAdditionalTrainingStart \\ \hline
    \parbox[c]{3cm}{\vspace{1mm} Additional Training\\ Experiment (Round 7) \vspace{1mm}} & \TPAdditionalTraining & \FPAdditionalTraining & \FNAdditionalTraining & \PrecisionAdditionalTraining & \RecallAdditionalTraining & \FScoreAdditionalTraining \\ \hline
    \hline
    \parbox[c]{3cm}{\vspace{1mm} Field Deployment \vspace{1mm}} & \TPFieldStudy & \FPFieldStudy & \FNFieldStudy & \PrecisionFieldStudy & \RecallFieldStudy & \FScoreFieldStudy \\
    \hline
\end{tabular}
\end{table*}

\JH{High-level comments: (1) suggest labeling each study as study 1, study 2, etc. and consistently referring to it in the text and tables. (2) For each study, clarify the goal, what the db setup was (clean or not), number of phones, etc. (3) For Table 1, suggest adding info about each study, ex. number of phones, number of traces, etc. (4) Section 5.2 needs more subsections, too long. (5) Evaluation needs better flow, seems like it jumps around. Start with an outline of key points, and then go from there.}

We evaluated \PP in four different contexts: a lab study, a small field study, a user survey from the field study, and a comparison of \PP with two other related systems - Recon \cite{ReCon} and Haystack \cite{HayStack}. 
%We present the results of four different evaluations, including a lab study, a small field study, a user survey from the field study, and a comparison against Recon \cite{ReCon} and Haystack \cite{HayStack}. 
Based on these evaluations, we highlight several key findings. First, we show that we can detect PII accurately with a precision of \PrecisionControlled and recall of \RecallControlled in the lab experiment and, a precision of \PrecisionFieldStudy and a recall of \RecallFieldStudy in the field study. 
%SK{Mention the number of users here for field study?}
% \YA{no recall numbers mentioned?} 
Second, we quantify the improvement in detection efficiency as the number of signatures (number of users using the same app) in our database increases. Third, \PP finds more PII than other approaches. Finally, based on our user survey, we show that \UsersWithNoBatteryLoss of the users in the survey found no perceptible change in battery life and \UsersWithNoNwPerformanceLoss users found no change in network performance. 

% \JH{Need to fix the third item to highlight more interesting parts}
% We published \PP on Google Play in Nov 2016. We also conducted an IRB-approved user study with 18 users over 4 days, which included an in-app survey to assess user awareness about privacy and the usability of \PP in terms of overhead, impact on other apps, and battery life. In the rest of this section, we first explain the experiment scenarios and design. We then present the results from our controlled experiments and user study. 
%\GS{Fixed it, Lets' be as specific as posssible}\SK{Should we be more specific with the dates or early/later is OK?} 


%\GS{Included}\YA{TODO: add a summary of what will come in this section}

% \YA{be more specific which sub section?} 

\vspace{-2mm}
\subsection{Experimental Design}
\vspace{-1mm}
For both the lab study and the small field study, we identified PII using the definition in Section \ref{sec:arch:identify}. We calculated Precision, Recall, and F1 scores by manually labeling each key-value pair as potential PII and then comparing against results from \PP. Note that an app might make many requests to the same host/path with the same key-value pair. If we analyze all these requests as separate events, then we will inflate the number of detected PII/non-PII key-value pairs in our experiments. To address this, we only examine unique (SID, key, value) tuples. 

% To combat this, we only include the value as detected PII in our experiment, if we have not seen another request with the same unique (SID, key, value) tuples. 
% The \PP server receives anonymized private signatures from the user's device while they use our Android app. Due to our privacy-sensitive design, we detect PII only on the user's device using their private signatures and public signatures from our crowdsourced signature DB. Hence, we use our test device (simulating a user) and then manually label the detected values as PII/non-PII to evaluate the detection efficiency. We use \PP app to extract key-value pairs from app requests for PII evaluation. 
%\GS{Addressed in the mail as well with Precision numbers.}\YA{I thought we only upload each unique signature once per app/user, why is this a problem?}. \GS{This is that since detection happens on the phone, if users opens an app 10 times, 10 times for ex. Android ID would be sent for same app, host. For TP and FP calculation on test device we will not consider 10 but we will consider this as 1}
%\SK{What if the SID is same, but value is different each time for the same key? This can happen with location, but you will only consider the first one location and ignore the rest unless you consider unique SID-key-value tuples. I think this is confusing. Also in the architecture section, it says C(S,k) is non-unique number of values. This indicates that it will count same values multiple times while the above para seems to indicate otherwise. - Fixed it}
%\GS{Check, if needed}In addition, every request in our analysis has a unique SID.

\textbf{Scenario 1: Controlled Experiment}: \KB{We selected the top \totalApps free apps from the Play Store for this experiment. Out of the \totalApps apps, we were only able to evaluate \totalAppsRunOnDroidbot apps. We found that \appswithCertificatePinning apps used certificate-pinning on all the network requests, \appswithLogin  required information such as bank accounts and phone numbers for account creation, and \appswithnonetwork made no network requests.} 
Each ``training run'' for an app consisted of installing the app, exploring it for 150 seconds and then uninstalling it. We used DroidBot \cite{DroidBot} to perform 4 training runs of each app on 4 Android Nexus-5X phones running Android 6.0 with \PP running in the background. Next, we used the same automated script on a fifth Nexus-5X phone running Android 6.0 as a ``test run'' to evaluate the results and the PIIs detected by \PP. While we configured Droidbot to interact with the apps in the same way across runs, there was still some variation due to non-deterministic behavior in apps,  variation in the environment, or timing issues. For instance, when Droidbot clicks a button, sometimes it successfully completes the desired function while at other times it fails due to slow network speeds. Similarly, Droidbot's interactions can differ as apps change the phone environment by turning on accessibility settings, changing the language of the phone, turning off the WiFi, and so on. To verify our results, we manually inspected each unique key-value pair that \PP extracted from the test run on the 5th device. 

\textbf{Scenario 2: \PP Field Deployment}: In this scenario, our signature database was created by users who installed our app from the Play Store and from our user study. We recruited 18 participants from an online portal, asking them to use \PP for at least 4 days. This was an IRB-approved User Study and participants were given a \$20 Amazon Gift Card. Participants were asked to keep \PP running for as long as possible and use their devices as they normally do. After 4 days, all participants were given the option to take a survey from the app. We also published the app on Google Play (published in Nov 2016) for organic users to discover the app on their own. The user study ran from Nov, 2016 to Jan, 2017. Then we ran the field study using organic users till May, 2017. 

We collected \totalPublicSignaturesFieldStudy signatures from \totalAppsFieldStudy apps. We took the top 100 apps based on signature count and installed them on a test device. The top five apps were BBC News, IMDb, MoneyControl, Pinterest, and Skout. We used a test device to evaluate \PP's PII detection accuracy, obviating the need for actual users to share their original key-value pairs. We manually launched these 100 apps and interacted with them for a minute on our test device. We then examined the key-value pairs marked by \PP as PII.
%\GS{We did Manual testing}\SK{Was the manual interaction done randomly? It may be better to clarify this as it can possibly introduce bias in the experiments.}
% pairon our test device that can leverage the signatures uploaded by crowd users to our signature DB. Then we extracted the list of key-value pairs detected by \PP as PII. 
We also collected telemetry information from users about the apps which were detected to leak PII. We got app package name, count of detected PII, count of user-marked PII and non-PII values, and the count of protocols (HTTP/ HTTPS/ Other) used by the app. This information enabled us to make decisions on whitelisting the apps on the server side.
%\JH{Was this info actually used to do pre whitelisting?} \GS{Yes, Slack currently comes as pre-whitelisted.}\KK{I suggest remove the telemetry part since it goes against the whole "privacy-sensitive" test design of using test devices, especially if pre-whiteliting was not actually done} \GS{Pre-Whitelisting is done. And the it does not violate privacy sensitive design because, we only collect counts, no actual value} \YA{keep this} %\GS{Included}\GS{Mention about telemetry here. In 1-2 lines. Part of experiment design} %\GS{Table \ref{tab:precision}}\YA{meta comment: we need this table asap.} %\GS{Included}\YA{Ideally we want to compare what our app finds for these apps and what Recon and Haystack find (or compare for a subset of these apps).} \GS{Table 1 I have done for one app, but it is taking alot of space, Any suggestion on representation of this.} %\GS{We install 100 apps which have most signatures in crowdsource DB on our test device}\YA{Meta comment 2: For this scenario, how do we get TP, FP, TN, FN?) These are the top 100 apps and 25 user apps no?}

%\vspace{-3mm}
\subsection{Detection Efficiency}
%\vspace{-1mm}

%\KB{Remove/Rephrase this (already talked about before): We manually labeled key-value pairs \PP classified as PII. We considered values such as unique identifiers to be true positives, and the rest false positives.} 
\KB{As mentioned earlier, unique key-value pairs for all of the network requests from the tests were marked manually to serve as the ground truth for the evaluations. This includes requests that did not meet the confidence threshold as well. Note that the labeling is an over approximation of false positives as some of these values might contain app-specific PII we were not aware of. We used a probability threshold of $T = \privateProbThreshold$ based on preliminary lab tests. The results of for both scenarios are shown in Table \ref{tab:precision}. }
%As described in Section \ref{sec:arch:identify}, the PII in Table \ref{tab:precision} are categorized into three confidence levels: High, Moderate and Low Likelihood. 

\textbf{Scenario 1:}\KB{
Our interactions in scenario 1 led to \totalPublicSignaturesControlled public signatures from the \totalAppsRunOnDroidbot apps out of \totalApps apps that we were able to evaluate. We then used another device to detect PII by interacting with the apps that had generated public signatures as described earlier. We labeled each of the \PIILeaksControlled unqiue key-value pairs collected from the test device. \PP marked \TPControlled True Positives, \FPControlled False Positives, \TNControlled True Negatives and \FNControlled False Negatives (Table \ref{tab:precision}).} Due to limitations of the automated testing framework, we cannot trigger all possible PII leaks from the apps. Therefore, we calculated the false negatives considering only the network requests we saw in our experiments. Interestingly, the Brightest Flashlight LED app transmitted the SHA hash of the UDID. Apps like Draw.ly, Drink Water Reminder, and Yelp used random hashes as identifiers for the device. In such scenarios, regex-based approaches can easily miss PII if we do not have a priori knowledge. Additionally, users may not have sufficient knowledge to label values like these as PII. Lastly, the current permission-based controls in Android would not be able to control such PII leaks.

% \KB{We observed that many of the False Positives marked as PII by \PP were because the system had not seen enough instances of the same network request. (Should we talk about how one instance means private probability will be 1?) We introduced a threshold for the number of times a request must be seen before \PP can begin identifying likely PIIs. This threshold can be configured by the users. (Refer to graph) shows the change is precision and recall with increasing threshold values. }
\NDSS{We observed that many of the false positives occur because \PP had not seen sufficient number of network requests for the same SID during the evaluation. We believe that as \PP observes more requests, its precision should increase. To test this hypothesis, we selected \totalAppsForMoreTraining apps with the most false positives in the controlled experiment and incrementally trained them for additional rounds to understand how the precision changes with more observations of network requests. This experiment was conducted separately, starting afresh from a clean database without using any data collected in the previous evaluation. In each round of this evaluation, we collected signatures by running the 4 training phones for 750 seconds each and recorded \PP 's precision and recall after each training round. We used the same training and testing devices for this experiment as well. The apps were not uninstalled at the end of each training round as in the controlled experiment. We collected signatures by running the test device for 750 seconds as well. To mitigate the non-determinism of the apps, we only observed the SIDs generated from the first round of this evaluation. The average precision slowly increases with more rounds of training as shown in Figure \ref{fig:PrecisionVsTraining1}. Evaluation of false positives after re-running these apps shows significant reduction in the number of false positives and an increase of overall precision of these \totalAppsForMoreTraining apps from \PrecisionAdditionalTrainingStart to \PrecisionAdditionalTraining.} 

\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{TrainingThreshold1}
  \caption{Precision and recall after 1 round of training}
  \label{fig:TrainingThreshold1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{TrainingThreshold2}
  \caption{Precision and recall after 7 rounds of training}
  \label{fig:TrainingThreshold2}
\end{subfigure}
\caption{Effect of the confidence threshold on the overall precision and recall of \PP after 1 round and 8 rounds of training. \textmd{The precision and recall is calculated for 40 apps with the most False Positives in the initial evaluation.}
}
\label{fig:TrainingThreshold}
\end{figure*}

\NDSS{We also conducted an experiment to understand the change in the performance of \PP's classification with varying levels of confidence threshold. The confidence threshold dictates the number of times a network request must be seen before \PP would start classifying it. Figure \ref{fig:TrainingThreshold2} shows the effect of confidence threshold value on precision and recall after 8 rounds of training. The precision increases and recall decreases as confidence threshold is increased. Based on the empirical data, the best threshold value is 2 for this experiment. Users can tune this threshold depending on how many false positives and false negatives they can tolerate. To further show the improvement due to additional training, Figure \ref{fig:TrainingThreshold1} shows the how the recall drops sharply while precision increases slowly with increased threshold after 1 round of training as compared to the 8 rounds of training.}

\KB{After manually analyzing the false positives found in the evaluation, we categorized them into four categories. First, \PP mistakenly detects some values as PII because in certain apps, the URL paths (which \PP uses as signature ID) had variable strings, e.g. \texttt{api.geo.kontagent.net/api/v1/} \newline \texttt{11828d55da4547b5b7bd85eef33c38a0/cpu/}. Since, these variable strings form a part of signature ID, \PP rarely sees enough instances of the request to classify it properly. Second, \PP is unable to correctly classify identifiers for objects on servers sent by the apps without sufficient number of users. Third, values which do not seem to have a semantic meaning but may or may not be PII. We label all such values as not PII is our ground truth. Finally, values belonging to network request made only one time. These values have a private probability of 1 and as discussed previously, \PP is unable to correctly classify such values without additional requests.}

\begin{figure}
\centering
\includegraphics[width=\columnwidth-10pt]{PrecisionVsTraining1}
\caption{Summary of change in precision of \PP with increasing number of training runs. \textmd{The precision numbers included are for the 20 apps which had the highest false positives in initial evaluation.}
}
\label{fig:PrecisionVsTraining1}
\end{figure}

%Graph for change in precision with number of users
% \begin{figure}
% \centering
% \includegraphics[width=\columnwidth-10pt]{AppCrowdUser}
% \caption{Summary of change in precision of \PP with increasing number of users. \textmd{The precision numbers included are for the set of 5 apps (Waplog, Pinterest, Moneycontrol, Smart Voice Recorder, and Yelp) used in this experiment. \SK{We can remove this if we don't have space}}
% %\GS{INcluded}\JH{Need to clarify, is this one app? Multiple apps? Also, label the x and y axes.}
% %\JH{Make the graph bigger, clip the whitespace on the edges.}
% }
% %\KK{Add ticks to the x-axis to indicate exact number of users} 
% \label{fig:ProgressivePrecision}
% \end{figure}


\textbf{Scenario 2:} Our crowdsourced DB was populated with the signatures from our user study and then by users who organically discovered our app on Google Play. In our crowdsourced DB, we had \SignCount signatures for 191 apps. In Scenario 2, we interacted with the top 100 apps with the most signatures, and captured requests for 75 apps, communicating with 30 remote hosts. 
%There are two reasons for why we only had data for 75 apps. \KB{Rephrase to talk about confidence threshold instead -- First, \PP signatures were not uploaded since the same network request was not seen 10 times in our use of apps for 1 minute. To reduce the number of False Positives, we designed \PP to only upload a signature to the server once it has seen the same network request at least 10 times.} \YA{why is it 10 here and 3 earlier?}
%Some apps require phone numbers to use, e.g. Marco Polo and Viber, and our device did not have this. 
\PP detected 116 potential PII leaks in 24 apps. We found 92 True Positives and 24 False Positives, resulting in a precision of 0.79 (see row 4 in Table \ref{tab:precision}). 

Analyzing the false positives, we noticed the News Break app retrieves news items by sending encoded URLs (e.g. \texttt{url:05QR8Z1i01}) similar to scenario 1 example. Different users read different news, so these key-value pairs were misclassified as PII. We found other  interesting cases of PII leaks, e.g. ``GO Weather Forecast \& Widgets'' sends IMEI to `t.appsflyer.com' (AppsFlyer), a mobile app tracking and attribution analytics library. The ``Gaana'' music app sends location to \texttt{`checkout.free} \newline \texttt{charge.in'} (payments app). Both are cases where PII use does not align with the purpose of the app. 
%\SC{New: Additionally, we manually ran \PP on 5 different phones with apps downloaded from BlackMart[cite], the app store to download paid apps for free. \PP detected that the versions of the apps found on this store had malware installed on them.}

%\SC{Gaurav, please write about the BLU phones.}
Crashlytics is a popular library for crash reporting and was detected by \PP to send (Android ID, Google AdID, Unique Installation ID, OS Build version) PII. This library was included in 24 apps (e.g. Skout, Tinder, Venmo) out of 191 apps in our signature DB. Interestingly, Crashlytics provides a feature on their web portal for developers so that users get a notification before sending a crash report (which contains PII). However, during our manual interactions with these apps we did not receive any such notifications, indicating that none of the developers enabled this feature.
% \GS{This should be crash report in place of PII. Should I change it. PII is a by-product of sending PII} \JH{I can't find CrashReport library 
%https://fabric.io/kits/ios/crashlytics?utm_campaign=crashlytics-marketing&utm_medium=natural}. 
% to get explicit consent from the users to share data with Crashlytics. 
%during our experiments as we manually interacted with these apps we did not receive any such notification. Hence its clear that the developer did not enable the privacy feature and did not take user's explicit consent to send data to Crashlytics.

The number of users for the 100 apps in scenario 2 ranged from 1 to 10 users. 54 apps had only 1 user, but 3 apps had 6 users (Moneycontrol, Airdroid, News Break), 1 app had 8 users (System App: Android Backup Service), and 1 app had 10 users (System App: Google Services Framework). 
% As shown in Table \ref{tab:precision}, we note that the precision improved significantly (34\%) in scenario 2 compared to scenario 1 although there were only 46 apps with more than 1 user.

%03 August 2018 - Removed due to space constraints
% \SK{Should we talk about this expt after our new expt on more training?} Our hypothesis is that detection accuracy would increase considerably as our user base increases. To test this, we designed another experiment where we simulated a progressive increase in the number of users. We started with 1 device and interacted with a set of five apps for a minute each (Waplog, Pinterest, Moneycontrol, Smart Voice Recorder, and Yelp). These five apps were selected randomly from the top 20 Apps used in Scenario 2. We then repeated the process on 5 more devices (6 total). Two devices were identical while the others were different Android smartphones. Figure \ref{fig:ProgressivePrecision} shows how PII detection (precision) changes as we add the number of devices using these 5 Apps ranging from 46\% for 1 device, to 70\% for 5 additional devices. Note that reported PII detection accuracy is achieved without users explicitly marking any values as PII. If we used that information, the precision numbers should be even better. This observation also applies to the Precision/Recall numbers presented in Table \ref{tab:precision} for Scenario 1 and Scenario 2. While our earlier experiment on 25 apps showed that precision of \PP improves when the apps are used more often, this experiment shows precision will also improve when \PP has more users.  \YA{I wonder if this is still useful given the other scenario 1 results of increasing precision? If we leave it, we should say that we can say with certainty based on both these experiments that precision does improve as we have more devices, as we expect. }
%We randomly selected these 5 downloaded apps from the top 20 apps from the 100 apps in Scenario 2. 
%\JH{list the apps, and why these apps? How selected?}
% \JH{identical devices? and 6 devices total?}.\GS{6 Devices. But not identical. Two of them were identical but not rest.} 
% \YA{new: please read.} 
%We note that these detection rates are currently based on a purely algorithmic approach. Again, \PP provides UIs for users to mark values to be filtered, helping us learn what keys are and are not PII. As such, false positives should go down considerably. Hence, we consider the presented precision values to be modest estimates.
%We measured the change in precision (see Figure \ref{fig:ProgressivePrecision}). We note that these detection rates are currently based on a purely algorithmic approach. Again, \PP provides UIs for users to mark values to be filtered, helping us learn what keys are and are not PII. As such, false positives should go down considerably. Hence, we consider the presented precision values to be modest estimates.
%There was bug in the Location detection code, Saksham has fixed it now, hence updating the numbers in the table. % YA: This comment is now handled I think. 
%\JH{I commented out the paragraphs about common keys. }
%\JH{Suggest give more info about basic statistics from Scenario 2, examples of true positives, etc. Plus, any other interesting tidbits, like apps that leak a lot. Maybe even manually inspect to see what kinds of PII is leaked, e.g. formats, and show that regex might not easily work for some unless you know to look for it beforehand. And show that permissions wouldn't really work either, as we argued in the intro.\GS{Address this specifically with example. Please review.} Lastly, should add something about effectiveness of filtering, ie did it break apps?}

%Table for approach comparision
\begin{table*}
\caption{
  Comparison of \PP, Recon, and HayStack in detecting unknown PII for 15 Apps that we analyzed. 
  \textmd{The first two rows present two example apps showcasing the ability of \PP to find non-standard PII as compared to other approaches. 
    \textsuperscript{1}We categorize false positives based on the strict definition of
    PII we use in this paper. For example, Gender and Time-Zone alone cannot 
    identify a person, though can if combined with other values, as discussed in
    Section \ref{sec:limitation}. }
   % \GS{Since Usenix provides extra space to provide appendices apart from 13 page limit, please add the detailed table of 15 apps as appendix and refer here so that we can defend nitpicking}
}
\label{tab:app_wise_comparision}

\small
\centering
\begin{adjustbox}{center, width=(\columnwidth-10pt) * 2}

\begin{tabular}{|c|c|c|c|c|}
\cline{1-5}
\textbf{Package Name} & \textbf{Metrics} & \textbf{Recon}            & \textbf{HayStack}                & \textbf{PrivacyProxy} \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}com.abtnprojects\\ .ambatana\end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering Advertiser ID, Device ID, Android ID, Email, Location} & 
\multicolumn{1}{|p{4cm}|}{\centering Android ID, Advertising ID, Hardware ID} & 
\multicolumn{1}{|p{5cm}|}{\centering Local IP, Device Fingerprint ID, First Launch Date, Advertiser ID, Identity ID, UID, Hardware ID, Google Advertising ID, Install Date}\\ \cline{2-5} 
 & \centering False Positives\textsuperscript{1} & {\centering -} & {\centering Build Fingerprint, Account Information} & {\centering Timestamp} \\ \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}tv.telepathic\\ .hooked\end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering Advertiser ID, Android ID}                   & 
\multicolumn{1}{|p{3cm}|}{\centering Android ID}                     & 
\multicolumn{1}{|p{5cm}|}{\centering Identity ID, Local IP, Device Fingerprint ID, Android ID, Hardware ID, Google Advertising ID, Identity ID, FirstLaunchDate, AppsFlyerID, UID, Session ID}
\\ \cline{2-5} 
 & \centering False Positives\textsuperscript{1} & {\centering -} &
{\centering  Build Fingerprint, Account Information} & \multicolumn{1}{|c|}{\centering Timestamp, Date} \\ \hline 

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} Total PII Count\\in the 15 apps \end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering 68}                   & 
37                     & 
\multicolumn{1}{|p{5cm}|}{\centering 96}
\\ \cline{2-5} 
 & \centering False Positives\textsuperscript{1} & {4} &
{\centering 21} & 22\\ \hline
\end{tabular}

\end{adjustbox}
\end{table*}

\textbf{Comparison with Recon and HayStack:} We also compared \PP's PII detection with Haystack \cite{HayStack} and Recon \cite{ReCon}. We collected the Top-100 apps from Google play store on July 31st, 2017 and then randomly selected 15 apps from this set for further testing. We tried to download and use Recon but were unable to get it to work for us. Therefore, we contacted the authors of Recon, and sent them the apks for these 15 apps for them to run their App on and send us the results of detected PIIs. We installed Lumen Privacy Monitor (HayStack) and reported results from their app for the set of these 15 test apps. We used the same device on the same network, and used HayStack and \PP one after the other to report PII flagged by them for these same 15 apps. For \PP, we used 5 phones to generate signature and then used another phone to evaluate. For brevity, we have included a few representative apps from our test setup in Table \ref{tab:app_wise_comparision} and we include the PIIs detected by those apps, as well as the total PIIs detected for all 15 apps. Our goal was to evaluate whether there are certain PII that approaches based on user supplied labeling (ReCon), and deep packet inspection (Haystack) would miss as compared to \PP or vice-versa. As noted in Table \ref{tab:app_wise_comparision}, \PP identified many more correct PII than either approach (True Positives). Considering true positives, \PP found 96 PII while Recon detected 68 PII and HayStack could find only 37 PII for these 15 apps. Being a more generic approach, \PP has more false positives than other two approaches while detecting more PII than other specialized approaches. 
% \YA{also, the data from the table shows that Recon also has lower FPs than us? Is that true? So, presumably while we find more PIIs, we may make it harder for the user?}
% \KB{We do increase the user burden slightly but isn't this issue mitigated by crowdsourcing the labeling?}
% \SK{Yes, \PP seem to have more FPs, but they should reduce with more training/users}

%\SC{We understand that PrivacyProxy works best for the apps for which \PP has the most signatures i.e. the most common apps being used by the user's of \PP. However, studies [cite Dohyun's paper] have shown that app usage has a long tail in terms of the apps being used. The majority (92\%) of the usage comes from the Top 3000 apps. To eliminate the bootstrapping issue with \PP, we ran a monkey[cite] on Top 3000 apps on 5 different phones and collected the signatures for these apps.}
%\SK{What is the significance/effect of the above on the results?}
% \YA{How many Apps did you test?
% \GS{10 apps from scenario 2, HayStack finds 12 TP and PP 31 TP} can we add a statement that PP always found more PII than them? 
% \GS{we can say that we found more than HayStack, in recon case I have to confirm for what we missed. But probably it could go a bit harsh comparison, i think the table already gives an idea.}}
% as compared to Recon and Haystack. \YA{new:read.} 
%Our results show that indeed, we detect many of the PIIs that both Haystack and Recon miss. The key idea for this evaluation was to evaluate if we would detect some unknown PII that would probably be missed by approaches relying on regex, deep packet inspection (DPI), or models based on user labeling PII or not \KK{what are user labels?} to predict likely PII. As the table shows we detect many of the values which are actually PII and missed by both the approaches.


\begin{table}

\caption{Summary of our findings from Request key analysis. \textmd{Analyzing the \totalPublicSignaturesFieldStudy signatures for \totalAppsFieldStudy apps from our crowdsourced signature database we found $~$31\% of apps leak at least one of the PII types.}}
\label{tab:AppKeyLibraryAnalysis}

\small
\centering
\begin{adjustbox}{center, width=\columnwidth-10pt}
\begin{tabular}{|c|c|} \hline
\multicolumn{1}{|p{5cm}|}{\centering \textbf{Type Of PII}
										\\(Based on Request Key)
                                     } &
\multicolumn{1}{|p{2.7cm}|}{\centering \textbf{Apps with corresponding PII} \\(Total Apps = 191) }\\ \hline \hline

\multicolumn{1}{|p{5cm}|}{\centering \textbf{Standard Identifiers (A)} 
										\\ (IMEI, Advertisement ID(AdID), Android ID, Crashlytics Install ID)
                                    	}
                                        & 
                                        \multicolumn{1}{|p{2.5cm}|}{\centering 57 \\29.8\%}
                                        \\ \hline

\multicolumn{1}{|p{5cm}|}{\centering \textbf{Location(B)} 
									   \\ (Latitude, Longitude, Zipcode)
                                       } & 
\multicolumn{1}{|p{2.7cm}|}{\centering 21 (11.0\%)}  \\ \hline

\multicolumn{1}{|p{5cm}|}{\centering \textbf{App Generated Unique Identifiers(C)}
										\\ (Device Fingerprint ID, Install ID, Identity ID, Attribution ID, Hardware ID, Placement ID ..)                                             } & 
\multicolumn{1}{|p{2.7cm}|}{\centering 19 (10.0\%)}  \\ \hline \hline

\multicolumn{1}{|p{5cm}|}{\centering \textbf{All categories above (A+B+C)}} & 
\multicolumn{1}{|p{2.7cm}|}{\centering 70 (36.7\%)}  \\ \hline

\hline
\end{tabular}
\end{adjustbox}

\end{table}


\textbf{Taxonomy of Keys containing PII:} Since our signatures are created using key-value pairs from the HTTP requests, it is possible to look for known PII (such as IMEI and Android ID) and identify all associated keys across different apps. For example, some of the keys associated with Android ID are \texttt{Android-ID,  X-CRASHLYTICS-ANDROID-ID, DeviceID}. Analyzing the \totalPublicSignaturesFieldStudy signatures for \totalAppsFieldStudy apps from the signature server database, we discovered that $~$31\% of apps leak at least one of the PII types (see Table \ref{tab:AppKeyLibraryAnalysis}). Furthermore, since many apps use the same libraries, we can potentially improve \PP's coverage for apps we have not seen before if they use keys known to be associated with PII leaks.

%\vspace{-4mm}
\subsection{\PP Usability}
%\vspace{-1mm}
%Since, we are doing the PII detection on the device itself, it is bound to negatively affect the battery life of the device. Apart from the display screen, the major battery drain in Smartphones is caused by the WiFi \cite{PathakEProfBattery}.
In Section \ref{sec:impl}, we discussed the various optimizations we did to reduce the energy overhead of running \PP, which we measured to be 30\% higher without our techniques. To quantify impact on battery life, we installed the top 20 apps from ``Free in Android Apps'' on our test devices. For the first test, we launched these apps (in the background) and then put the device in standby mode (screen off). In the second test, we used the MonkeyRunner script to open each of these 20 apps one by one, and interacted with them by performing 100 clicks on the screen (screen is on in this case). To measure overhead, we calculated the time it took for the battery to go from from 100\% to 85\% with and without \PP enabled. Note, to mimic typical user settings, we enabled the WiFi radio, LocationServices, etc on the test device and ran each test thrice to report data. Table \ref{tab:table_batterylife} presents the energy overhead results. Our data shows that for standby, \PP reduces battery lifetime by 9.7\% - 11.0\%, while in active use the overhead can be up to 14.2\%. Past work found that VPNs can consume nearly 10\% battery by themselves \cite{rao2013meddle}, so the additional battery consumption due to \PP parsing and filtering appears to be minimal.

\begin{table}
  	\caption{Battery Overhead Evaluation. \textmd{The percentage depicts the reduction in battery life, which varied from 12.8\% to 14.2\% in our 2 test devices.}}
\label{tab:table_batterylife}
\small
\begin{tabular}{|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Scenario}}}                      & \multicolumn{2}{l|}{\textbf{Samsung S7 Edge}}                                                                            & \multicolumn{2}{l|}{\textbf{Nexus 5X}}                                                                                 \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                        & \textbf{Standby}                                            & \textbf{Monkey}                                            & \textbf{Standby}                                           & \textbf{Monkey}                                           \\ \hline
\begin{tabular}[c]{@{}l@{}}Without\\ PrivacyProxy\end{tabular}                & 463 min                                                     & 52 min                                                     & 650 min                                                    & 70 min                                                    \\ \hline
\begin{tabular}[c]{@{}l@{}}With \\ PrivacyProxy\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}416 min \\ (10.2\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}46 min \\ (11.5\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}594 min \\ (8.6\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}61 min\\ (12.8\%)\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}With\\  PrivacyProxy \\ and Filtering\end{tabular} & \begin{tabular}[c]{@{}l@{}}412 min\\ (11.0\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}45 min \\ (13.4\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}587 min \\ (9.7\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}60 min\\ (14.2\%)\end{tabular} \\ \hline
\end{tabular}
    
% %\small
% \footnotesize
%   \begin{tabular}{|l|l|l|l|l|}
%     \hline
	
%     \multicolumn{1}{|p{1.8cm}|}{\centering \textbf{Scenario}} &
%     \multicolumn{2}{|c|}{\textbf{Samsung S7 Edge}} & \multicolumn{2}{|c|}{\textbf{Nexus 5x}}  \\ \cline{2-5}
    
%      	 & \textbf{StandBy} & \multicolumn{1}{|p{1cm}|} {\centering \textbf{Monkey Runner}} & 
%          \textbf{StandBy} & \multicolumn{1}{|p{1cm}|} {\centering \textbf{Monkey Runner}} \\
%     \hline \hline
%     \multicolumn{1}{|p{1.7cm}|}{\centering Without PrivacyProxy } & 
%     	\multicolumn{1}{|p{1cm}|} {\centering 463 min} &
%     	\multicolumn{1}{|p{1cm}|} {\centering 52 min} &
%         \multicolumn{1}{|p{1cm}|} {\centering 650 min} &
%         \multicolumn{1}{|p{1cm}|} {\centering 70 min} \\
%     \hline
%     \multicolumn{1}{|p{1.7cm}|}{\centering With PrivacyProxy } & 
%     	\multicolumn{1}{|p{1cm}|} {\centering 416 min 	\\10.2\%} &
%     	\multicolumn{1}{|p{1cm}|} {\centering 46 min 		\\11.5\%} &
%         \multicolumn{1}{|p{1cm}|} {\centering 594 min 	\\8.6\%} &
%         \multicolumn{1}{|p{1cm}|} {\centering 61 min 		\\12.8\%} \\
%     \hline
%     \multicolumn{1}{|p{1.7cm}|}{\centering With PrivacyProxy and Filtering } & 	 		
%     	\multicolumn{1}{|p{1cm}|} {\centering 412 min 	\\11.0\%} &
% 	  	\multicolumn{1}{|p{1cm}|} {\centering 45 min 		\\13.4\%} &
%         \multicolumn{1}{|p{1cm}|} {\centering 587 min 	\\9.7\%} &
%         \multicolumn{1}{|p{1cm}|} {\centering 60 min 		\\14.2\%} \\
%     \hline
% \end{tabular}

% \vspace{-3mm}
\end{table}
%and we are investigating optimizations to reduce the overhead further.

% Since the dominant state of most users' devices is in standby, we believe the overheads are acceptable although we are investigating techniques to reduce this overhead further.
% \SC{included \KK{To make the comparison meaningful both tests should have the screen on at the same brightness. screen takes up a lot of battery}}

% SC{included} \KK{Are the screens on during the test? How about WiFi etc?}
%\KK{\GS{It should be Overhead}unclear what this means. 30\% faster than without \PP?}
%\SC{included. Running tests now}\YA{This is for the non-interactive case? i.e. you launch some apps and then let them run in the background with the screen turned off correct? We would need to make the case why we don't evaluate during regular usage (maybe because its hard to replicate?).} 

 
%\subsection{User Survey} 
\label{sec:user_survey}
% Additionally, 7 users downloaded \PP from Play Store and took the same survey without explicit requirement.

% The participants were asked to keep \PP running for as long as possible and use their devices as they normally do. After 3 days, the option to take the Survey was available and the participants were asked to take the Survey from the app.

%\JH{Is there a Google doc somewhere of the survey results? Will be easier if I can see that too. Need to describe the questions and the scale. Need enough details for others to replicate.}

%CBDR (for anonymity).
% So our users are probably more tech savvy than the average mobile user.

We conducted an in-app user survey to measure perceived usability and performance overhead of \PP. The survey was delivered after 3 days of using \PP. All questions were on a 5-point Likert scale. 
For battery consumption, 85\% (23/27) of survey participants said that they ``Noticed no perceptible change''. 67\% (18/27) said the same about network performance. Although there is a performance overhead of using \PP, 54\% (14/26) of participants agreed that the performance overhead was worth the privacy improvement while 31\% (8/26) were neutral. Overall, 59\% (16/27) of users were able to use \PP without noticing any perceptible change to apps. 

==> old_files/05_evaluation_old.tex <==
\section{Evaluation}
\label{sec: Evaluation}

% Table for Precision PI Detection
\begin{table*}
\centering
\begin{adjustbox}{center, width=(\columnwidth-10pt) * 2}
%\label{tab:precision}
\begin{tabular}{|cc|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c}{\textbf{Scenario}} & &\textbf{Confidence Level}& \multicolumn{1}{c|}{\textbf{TP}} & \multicolumn{1}{c|}{\textbf{FP}} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\ \hline \hline

\multirow{4}{3cm}{Controlled Experiment (Scenario 1)} & \multicolumn{1}{c|}{43} & \multicolumn{1}{c|}{27} & 0 & 0.61 & 1.0 & 0.76 \\ \cline{3-9} 
                                    & 15                      & 27                      & 1 & 0.36 & 0.94 & 0.52 \\ \cline{3-9} 
                                    & 2                       & 15                      & 1 & 0.12 & 0.67 & 0.20 \\ \cline{3-9} 

& \multicolumn{1}{c|}{Overall} & 82                      & 58                      & 1 & 0.59 & 0.99 & 0.74 \\ \hline

\multirow{4}{3cm}{\PP in wild and User Study (Scenario 2)}   & 5 & Highly Likely                & \multicolumn{1}{c|}{51} & \multicolumn{1}{c|}{11} & 0 & 0.82 & 0.90 & 0.89 \\ \cline{3-9} 
                                   & 6  & Moderately Likely      		& 39                      & 10                      & 0 & 0.80 & 1.0 & 0.89 \\ \cline{3-9} 
                                   & 7  & Less Likely          		& 2                       & 3                       & 0 & 0.40 & 1.0 & 0.57 \\ \cline{3-9} 
                                  & 8   & \multicolumn{1}{c|}{Overall} & 92                      & 24                      & 0 & 0.79 & 1.0 & 0.88 \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Summary Table showing detection efficiency in controlled experiment and in wild and user study. \textmd{The precision rates in our controlled experiment are relatively low although we see from the results of the Scenario 2 as the number users increase the precision improved by 34\%.}}
\label{tab:precision}
\end{table*}


We evaluated \PP in four different contexts: a lab study, a small field study, a user survey from the field study, and a comparison of \PP with two other related systems - Recon \cite{ReCon} and Haystack \cite{HayStack}. 
%We present the results of four different evaluations, including a lab study, a small field study, a user survey from the field study, and a comparison against Recon \cite{ReCon} and Haystack \cite{HayStack}. 
Based on these evaluations, we highlight several key findings. First, we show that we can detect PII accurately with a precision (\PrecisionScenarioA) and recall (0.99) in our lab experiment and precision (\PrecisionScenarioB) and recall (1.0) for our field study. 
%SK{Mention the number of users here for field study?}
% \YA{no recall numbers mentioned?} 
Second, we quantify the improvement in detection efficiency as the number of signatures (number of users using the same app) in our database increases. \YA{say what it improves to? is this changing the precision of 0.61 to 0.85?} Finally, based on our user survey, we show that 85\% of the users in the survey found no perceptible change in battery life and 68\% users found no change in network performance. 

% \JH{Need to fix the third item to highlight more interesting parts}
% We published \PP on Google Play in Nov 2016. We also conducted an IRB-approved user study with 18 users over 4 days, which included an in-app survey to assess user awareness about privacy and the usability of \PP in terms of overhead, impact on other apps, and battery life. In the rest of this section, we first explain the experiment scenarios and design. We then present the results from our controlled experiments and user study. 
%\GS{Fixed it, Lets' be as specific as posssible}\SK{Should we be more specific with the dates or early/later is OK?} 


%\GS{Included}\YA{TODO: add a summary of what will come in this section}

% \YA{be more specific which sub section?} 

\subsection{Experimental Design}
We evaluated \PP in a lab study and a small field study, described below. For both studies, we identified PII using the definition in Section \ref{sec:arch:identify}. 
We calculated Precision, Recall, and F1 scores by manually labeling values as potential PII and then comparing against results from \PP. Note that an app might make many requests to the same host/path with the same key-value pair. If we analyze all these requests as separate events, then we will inflate the number of detected PII/non-PII key-value pairs in our experiments. To address this, we only examine unique (SID, key, value) tuples. 
%\JH{Double check that the unique part above is right, I tried to shorten things}

% To combat this, we only include the value as detected PII in our experiment, if we have not seen another request with the same unique (SID, key, value) tuples. 
% The \PP server receives anonymized private signatures from the user's device while they use our Android app. Due to our privacy-sensitive design, we detect PII only on the user's device using their private signatures and public signatures from our crowdsourced signature DB. Hence, we use our test device (simulating a user) and then manually label the detected values as PII/non-PII to evaluate the detection efficiency. We use \PP app to extract key-value pairs from app requests for PII evaluation. 
%\GS{Addressed in the mail as well with Precision numbers.}\YA{I thought we only upload each unique signature once per app/user, why is this a problem?}. \GS{This is that since detection happens on the phone, if users opens an app 10 times, 10 times for ex. Android ID would be sent for same app, host. For TP and FP calculation on test device we will not consider 10 but we will consider this as 1}
%\SK{What if the SID is same, but value is different each time for the same key? This can happen with location, but you will only consider the first one location and ignore the rest unless you consider unique SID-key-value tuples. I think this is confusing. Also in the architecture section, it says C(S,k) is non-unique number of values. This indicates that it will count same values multiple times while the above para seems to indicate otherwise. - Fixed it}
%\GS{Check, if needed}In addition, every request in our analysis has a unique SID.

\vspace{3mm}

\textbf{Scenario 1: Controlled Experiment}: We installed the top 100 apps from the ``Free in Android Apps" category on Google Play. For this experiment, the devices were allowed to upload the signatures after just 1 observation (as opposed to 10 in the usual deployment). We manually interacted with each app for 1 minute on an  Android device with \PP running in the background. Then, we repeated the same process on a different device to get more signatures. Afterward, we interacted with the same apps again on the first device and examined the results. 
% \KK{Sounds like there are 3 devices involved here? Also, it would be good to clarify that the experiment setup allowed client to upload signature after just 1 observation (as opposed to 10 in the usual deployment)}
% \YA{what do you mean? the 2nd device is also sending private signatures right}\GS{But since test scenario as soon as 1st request is made it will pull public sig for that SID and detect PII. The generated private sig will be uploaded later when uploader runs. This would be true for all requests.} 
Note that the two devices used were identical (unmodified Nexus 6P phones running Android 6.0.1), since if we used 2 different models, \PP might erroneously treat the model number or OS version as PII. To verify our results, we manually inspected each unique key-value pair the proxy extracted.
% \JH{Just double checking, the database was cleared, so there's only signatures from one device, is that right?} 
% \GS{Yes. So new DB and Server started at a different port to talk to this new DB}

\textbf{Scenario 2: \PP Field Deployment}: In this scenario, our signature database is created by users who installed our app from the Play Store and from our user study. Nine users found and downloaded \PP from Google Play (published in Nov 2016). We also recruited 18 participants from an online portal, asking them to use \PP for at least 4 days. This was an IRB-approved User Study and participants were given a \$20 Amazon Gift Card. Participants were asked to keep \PP running for as long as possible and use their devices as they normally do. After 4 days, all participants were given the option to take a survey from the app.
% \JH{Numbers don't match up, there are 7 + 18 users here, but the survey says 26 users} 
% \YA{check this?} 
% \SC{Some survey questions were not compulsory. Updated the number of users as 27 (18+9) everywhere}

We collected \totalSignatures signatures from \totalApps apps. We took the top 100 apps based on signature count and installed them on a test device. The top five apps were BBC News, IMDb, MoneyControl, Pinterest, and Skout.
%\JH{Good if you can list the top 5 apps, just to give readers a sense of things}
We used a test device to evaluate \PP's PII detection accuracy, obviating the need for actual users to share their original key-value pairs. 
%Using a test device to evaluate \PP's efficacy has the advantage that we do not require users who participated in our study to upload their private signatures, hence limiting any privacy concerns.
We manually launched these 100 apps and interacted with them for a minute on our test device. We then examined the key-value pairs marked by \PP as PII.
\SK{Was the manual interaction done randomly? It may be better to clarify this as it can possibly introduce bias in the experiments.}
% \YA{new, read}
% pairon our test device that can leverage the signatures uploaded by crowd users to our signature DB. Then we extracted the list of key-value pairs detected by \PP as PII. 

We also collected telemetry information from users about the apps which were detected to leak PII. We got app package name, count of detected PII, count of user-marked PII and non-PII values, and the count of protocols (HTTP/ HTTPS/ Other) used by the app. This information enabled us to make decisions on whitelisting the apps on the server side.
%\JH{Was this info actually used to do pre whitelisting?} \GS{Yes, Slack currently comes as pre-whitelisted.}\KK{I suggest remove the telemetry part since it goes against the whole "privacy-sensitive" test design of using test devices, especially if pre-whiteliting was not actually done} \GS{Pre-Whitelisting is done. And the it does not violate privacy sensitive design because, we only collect counts, no actual value} \YA{keep this}

%\GS{Included}\GS{Mention about telemetry here. In 1-2 lines. Part of experiment design}

%\GS{Table \ref{tab:precision}}\YA{meta comment: we need this table asap.}

%\GS{Included}\YA{Ideally we want to compare what our app finds for these apps and what Recon and Haystack find (or compare for a subset of these apps).} \GS{Table 1 I have done for one app, but it is taking alot of space, Any suggestion on representation of this.}

%\GS{We install 100 apps which have most signatures in crowdsource DB on our test device}\YA{Meta comment 2: For this scenario, how do we get TP, FP, TN, FN?) These are the top 100 apps and 25 user apps no?}

\vspace{-2mm}
\subsection{Detection Efficiency}
We manually labeled key-value pairs \PP classified as PII. We considered values such as unique identifiers and location true positives, and the rest false positives. Note that this is an over approximation of false positives as some of these values might contain app-specific PII we were not aware of. We also inspected potential PII values that were below threshold and hence not classified as PII, labeling these as false negatives. We used a threshold of $T = 0.6$ based on preliminary lab tests. The results of for both scenarios are shown in Table \ref{tab:precision}. As described in Section \ref{sec:arch:identify}, the PII in Table \ref{tab:precision} are categorized into three confidence levels: High, Moderate and Low Likelihood. 
% \YA{new:read}.
%based on how different the Private and Public signatures are. % YA: removed this sentence, but can add if unclear

\textbf{Scenario 1:}
Our interactions in scenario 1 led to 989 signatures. We then used the second device to detect PII by interacting with the same apps again. We captured requests from 40 apps, which communicated with 39 remote servers. The other 60 apps did not connect to any remote servers. \PP detected 140 potential PII leaks for 23 apps. We labeled the detected PII and calculated True Positive (82), False Positive (58) and False Negative (1) numbers (see row 4 in Table \ref{tab:precision}). 
% \YA{refer to table and mark rows in it.} %\JH{Good if you can give an example of an app that leaked a lot of PII, plus examples of PII.} 
Note that precision is highest for highly likely PII and decreases as our confidence decreases.

Interestingly, GO Weather Forecast and Widgets app (14 True Positives) generated two unique ids. One concatenates install time and Android ID (\texttt{14810493757127} \texttt{cfc44f05470b61a}). 
% and sends them to their servers (`goweatherex.3g.cn'). 
The other is a device fingerprint \newline \texttt{(deviceFingerPrintId:ffffffff-9333-3215-0000-} \newline
\texttt{000049eee8b9)}. These examples suggest regex-based approaches can easily miss PII if we do not have a priori knowledge. Additionally, users may not have sufficient knowledge to label values like these as PII. Lastly, the current permission-based controls in Android would not be able to control such PII leaks. 
% \SL{Update the examples}

% \JH{what app had this FN below?}\GS{SKOUT}
The only false negative was from Skout, which embedded multiple key-values inside of a single string value \texttt{("userid":112498803,}  \texttt{"datetime":1481051772274,} \texttt{"action":"Click")}. \PP marked this value as ``Context-Sensitive'' since the timestamp makes the string different across different users. The developer put multiple items in a single string, so \PP did not detect \texttt{userid}. This app was the only one we saw using this app encoding, where various key-value pairs are sent as a value inside another key. 
%This key had a private probability of 0.14 and public probability of 0.0. \PP marked this value as ``Context-Sensitive'' as the Private Probability is less than the threshold (0.6). \KK{Removed the probability part since that is not very intuitive why the public probability is 0 and doesn't contribute to the point that we're making (develoepr putting everything in 1 string)}
% \YA{Gaurav, check if this resolves the comment.} 
% \JH{Why public probability of 0? Is it that the signature didn't upload b/c it was below threshold??}
% \GS{The public probability is 0 because there is only one other user in this scenario, and hence even if the signature is there if we query the count-min sketch it will say it has not seen the value. (Because it has actually not seen the value). The reason it is flagged as non-PII is because it not see frequently in User's own request and hence the threshold is not reached. and we only interacted for 1 min so it did not make multiple request with same key.}
% \JH{Also, it didn't detect this b/c it's a long string that stuffs a lot of info in it?}

%\PP would detect this value as ``Context-Sensitive'' as the Private Probability is less than the threshold (0.6). Note that the classification is true in this case, as we see `Timestamp', and User Action(`Click') in the value, but since the developer put the \texttt{userid} in same key-value pair, \PP did not detect the `userid'. 


% \KK{Why do we need this specific example?} 
% \GS{This is not example. This is the 1 which is mentioned in the table \ref{tab:precision} detected during lab test.}
%\KK{why only 40?\GS{Only 40 used internet. I opened all 100 apps atleast once.}}
%\SK{How are splitting the key-value pairs and deciding which are keys, which are values? I thought that user\_id, datetime and action will become 3 keys instead of combining them into 1 key.}\GS{Ideally it should. That's what I have said in the text that the developer has put everyting in one key ``message\_message". This is a example of App specific encoding that developer is using}

%Table for approach comparision
\begin{table*}
\small
\centering
\begin{adjustbox}{center, width=(\columnwidth-10pt) * 2}

\begin{tabular}{|c|c|c|c|c|}
\cline{3-5}

\multicolumn{2}{c|}{} & Recon            & HayStack                & PrivacyProxy \\ 
\hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Waplog\\ com.waplog.social\end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering Username\textsuperscript{2}, Password, Tracking identifier (Android ID)}                   & 
Android ID                      & 
\multicolumn{1}{|p{6.5cm}|}{\centering Android ID, Latitude, Longitude, Google Advertising ID (Also sent as Advertising ID and IDFA), Crashlytics Installation ID, App/Library Specific IDs (Device Fingerprint ID, Hardware ID, Attribution ID, Identity ID, Generated ID,  Placement ID)}
\\ \cline{2-5} 
 & \centering False Positives\textsuperscript{1} & \multicolumn{1}{c|}{Gender} &
\multicolumn{1}{|p{2.6cm}|}{Time-Zone, Build Number} & Timestamp, Screen Resolution, Build Number\\ \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pinterest\\ com.pinterest\end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering Tracking identifier (Android ID)}                   & 
Android ID                      & 
\multicolumn{1}{|p{6.5cm}|}{\centering Android ID, Pinterest Install ID}
\\ \cline{2-5} 
 & \centering False Positives\textsuperscript{1} & \multicolumn{1}{c|}{-} &
\multicolumn{1}{|p{2.6cm}|}{Hardware Info, Build Fingerprint} & Event Timestamp \\ \hline

% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Total PII Count\\in Other Apps\end{tabular}} & True Positives  & \multicolumn{1}{|p{3cm}|}{\centering 20}                   & 
% \SC{16}                     & 
% \multicolumn{1}{|p{6.5cm}|}{\centering \SC{20..}}
% \\ \cline{2-5} 
%  & \centering False Positives\textsuperscript{1} & \multicolumn{1}{c|}{\SC{\_}} &
% \multicolumn{1}{|p{2.6cm}|}{\centering \SC{20..}} & \SC{10}\\ \hline

\end{tabular}

\end{adjustbox}
\caption{
  Comparison of \PP, Recon, and HayStack in detecting unknown PII.
  \textmd{
    \textsuperscript{1}We categorize false positives based on the strict definition of
    PII we are using for this paper. For example, Gender and Time-Zone alone cannot 
    identify a person, though can if combined with other values, as discussed in
    Section \ref{sec:limitation}.
    \textsuperscript{2}\PP did not flag \texttt{username} because the
    Waplog app put the \texttt{Username} in the URL path rather than query parameter.}
}

\label{tab:app_wise_comparision}
\end{table*}

\begin{figure}
\centering
\includegraphics[width=\columnwidth-10pt]{AppCrowdUser}
\caption{Summary of change in precision of \PP with increasing number of users. \textmd{The precision numbers included are for the set of 5 apps (Waplog, Pinterest, Moneycontrol, Smart Voice Recorder and Yelp) used in this experiment.}
%\GS{INcluded}\JH{Need to clarify, is this one app? Multiple apps? Also, label the x and y axes.}
%\JH{Make the graph bigger, clip the whitespace on the edges.}
}
%\KK{Add ticks to the x-axis to indicate exact number of users} 
\label{fig:ProgressivePrecision}
\vspace{2mm}
\end{figure}

\textbf{Scenario 2:} Our crowdsourced DB had \SignCount signatures for \totalApps apps. In Scenario 2, we interacted with the top 100 apps with the most signatures, and captured requests for 75 apps, communicating with 30 remote hosts. There are two reasons for why we only had data for 75 apps. First, our use of apps for 1 minute did not always reach the threshold of 10 observations before uploading. Second, some apps require phone numbers to use, e.g. Marco Polo and Viber, and our device did not have this. \PP detected 116 potential PII leaks in 24 apps. We found 92 True Positives and 24 False Positives, resulting in a precision of 0.79 (see row 8 in Table \ref{tab:precision}). 
Analyzing the false positives, we noticed the New Break app retrieves news items by sending encoded URLs (e.g. \texttt{url:05QR8Z1i01}). Different users read different news, so these key-value pairs were misclassified as PII. We found other  interesting cases of PII leaks, e.g. ``GO Weather Forecast \& Widgets'' sends IMEI to `t.appsflyer.com' (AppsFlyer), a mobile app tracking and attribution analytics library. The ``Gaana'' music app sends location to `checkout.freecharge.in' (payments app). Both are cases where PII use does not align with the purpose of the app. 
% \JH{Suggest discussing some TPs and FPs here.} 
% \YA{also refer to the table and the row in it} 


%\SC{New: Additionally, we manually ran \PP on 5 different phones with apps downloaded from BlackMart[cite], the app store to download paid apps for free. \PP detected that the versions of the apps found on this store had malware installed on them.}

%\SC{Gaurav, please write about the BLU phones.}

Crashlytics is a popular library for crash reporting and was detected by \PP to send (Android ID, Google AdID, Unique Installation ID, OS Build version) PII. This library was included in 24 apps (e.g. Skout, Tinder, Venmo) out of \totalApps apps in our signature DB. Interestingly, Crashlytics provides a feature on their web portal for developers so that users get a notification before sending a crash report (which contains PII). However, during our manual interactions with these apps we did not receive any such notifications, indicating that none of the developers enabled this feature.
% \GS{This should be crash report in place of PII. Should I change it. PII is a by-product of sending PII} \JH{I can't find CrashReport library 
%https://fabric.io/kits/ios/crashlytics?utm_campaign=crashlytics-marketing&utm_medium=natural}. 
% to get explicit consent from the users to share data with Crashlytics. 
%during our experiments as we manually interacted with these apps we did not receive any such notification. Hence its clear that the developer did not enable the privacy feature and did not take user's explicit consent to send data to Crashlytics.


% \SC{Updated numbers}

%The number of users for the 100 apps in scenario 2 ranged from 1 to 10 users. 54 apps had only 1 user, but 3 apps had 6 users (Moneycontrol, Airdroid, News Break),
%1 app had 8 users (System App: Android Backup Service), and 1 app had 10 users (System App: Google Services Framework). With the results from Table \ref{tab:precision} we note that the precision improved significantly (34\%) although there were only 46 apps with more than 1 user.
%\SC{Why does Google Services Framework appear in just 8, 10 users especially If they are part of the system?}

The number of users for the 100 apps in scenario 2 ranged from 1 to 10 users. 54 apps had only 1 user, but 3 apps had 6 users (Moneycontrol, Airdroid, News Break), 1 app had 8 users (System App: Android Backup Service), and 1 app had 10 users (System App: Google Services Framework). As shown in Table \ref{tab:precision}, we note that the precision improved significantly (34\%) in scenario 2 compared to scenario 1 although there were only 46 apps with more than 1 user.

Our hypothesis is that detection accuracy would increase considerably as our user base increases. To test this, we designed another experiment where we simulated a progressive increase in the number of users. We started with 1 device and interacted with a set of five apps for a minute each (Waplog, Pinterest, Moneycontrol, Smart Voice Recorder and Yelp). These five apps were selected randomly from the top 20 Apps used in Scenario 2.  
%We randomly selected these 5 downloaded apps from the top 20 apps from the 100 apps in Scenario 2. 
%\JH{list the apps, and why these apps? How selected?}
We then repeated the process on 5 more devices (6 total). Two devices were identical while the others were different Android smartphones. 
% \JH{identical devices? and 6 devices total?}.\GS{6 Devices. But not identical. Two of them were identical but not rest.} 

Figure \ref{fig:ProgressivePrecision} shows how PII detection (precision) changes as we add the number of devices using these 5 Apps ranging from 0.46 for 1 device, to 0.7 for 5 additional devices. Note that reported PII detection accuracy is achieved without users explicitly marking any values as PII. If we used that information, the precision numbers should be even better. This observation also applies to the accuracy (Precision/Recall) numbers presented in Table \ref{tab:precision} for Scenario 1 and Scenario 2. 
% \YA{new: please read.} 
%We note that these detection rates are currently based on a purely algorithmic approach. Again, \PP provides UIs for users to mark values to be filtered, helping us learn what keys are and are not PII. As such, false positives should go down considerably. Hence, we consider the presented precision values to be modest estimates.

%We measured the change in precision (see Figure \ref{fig:ProgressivePrecision}). We note that these detection rates are currently based on a purely algorithmic approach. Again, \PP provides UIs for users to mark values to be filtered, helping us learn what keys are and are not PII. As such, false positives should go down considerably. Hence, we consider the presented precision values to be modest estimates.
%There was bug in the Location detection code, Saksham has fixed it now, hence updating the numbers in the table.

% YA: This comment is now handled I think. 
%\JH{I commented out the paragraphs about common keys. }
%\JH{Suggest give more info about basic statistics from Scenario 2, examples of true positives, etc. Plus, any other interesting tidbits, like apps that leak a lot. Maybe even manually inspect to see what kinds of PII is leaked, e.g. formats, and show that regex might not easily work for some unless you know to look for it beforehand. And show that permissions wouldn't really work either, as we argued in the intro.\GS{Address this specifically with example. Please review.} Lastly, should add something about effectiveness of filtering, ie did it break apps?}


\textbf{Comparison with Recon and HayStack:} We also compared \PP's PII detection with Haystack \cite{HayStack} and Recon \cite{ReCon}. We installed Lumen Privacy Monitor (HayStack) on December 5\textsuperscript{th} 2016 and reported results from their app. We were unable to use Recon and so used data from Recon Reports \cite{ReconReport}. We used the same device on the same network, and used HayStack and \PP one after the other to report PII flagged by them for 10 apps from scenario 2. For brevity, we have included a few representative apps from our test setup in Table \ref{tab:app_wise_comparision} and we include the total PII detected by those apps. Our goal was to evaluate whether there are certain PII that approaches based on regex matching (PrivacyGuard), user supplied labeling (ReCon), and deep packet inspection (Haystack) would miss as compared to \PP or vice-versa. \SK{Where is the data of comparison with PrivacyGuard?} \KK{If we don't have data to compare against PrivacyGuard, we can note that their paper only provides regex for location, phone state (IMEI), and contact (email, phone number)} As noted in table \ref{tab:app_wise_comparision}, \PP identified many more correct PIIs than either approach (True Positives), but also has some false positives. Considering true positives, \PP found 31 PIIs while HayStack could find only 12 PIIs for these 10 apps.

% \KK{I don't think we compared against PrivacyGuard?}

%\SC{We understand that PrivacyProxy works best for the apps for which \PP has the most signatures i.e. the most common apps being used by the user's of \PP. However, studies [cite Dohyun's paper] have shown that app usage has a long tail in terms of the apps being used. The majority (92\%) of the usage comes from the Top 3000 apps. To eliminate the bootstrapping issue with \PP, we ran a monkey[cite] on Top 3000 apps on 5 different phones and collected the signatures for these apps.}
%\SK{What is the significance/effect of the above on the results?}

% \YA{How many Apps did you test?
% \GS{10 apps from scenario 2, HayStack finds 12 TP and PP 31 TP} can we add a statement that PP always found more PII than them? 
% \GS{we can say that we found more than HayStack, in recon case I have to confirm for what we missed. But probably it could go a bit harsh comparison, i think the table already gives an idea.}}
% as compared to Recon and Haystack. \YA{new:read.} 
%Our results show that indeed, we detect many of the PIIs that both Haystack and Recon miss. The key idea for this evaluation was to evaluate if we would detect some unknown PII that would probably be missed by approaches relying on regex, deep packet inspection (DPI), or models based on user labeling PII or not \KK{what are user labels?} to predict likely PII. As the table shows we detect many of the values which are actually PII and missed by both the approaches.


\begin{table}
\small
\centering
\begin{adjustbox}{center, width=\columnwidth-10pt}
\begin{tabular}{|c|c|} \hline
\multicolumn{1}{|p{4.9cm}|}{\centering Type Of PII
										\\(Based on Request Key)
                                     } &
\multicolumn{1}{|p{2.8cm}|}{\centering Apps with corresponding PII \\(Total Apps = \totalApps)} \\ \hline

\multicolumn{1}{|p{4.9cm}|}{\centering \textbf{Standard Identifiers (A)} 
										\\ (IMEI, Advertisement ID(AdID), Android ID, Crashlytics Install ID)
                                    	}
                                        & 
                                        \multicolumn{1}{|p{2.5cm}|}{\centering 57 \\29.8\%}
                                        \\ \hline

\multicolumn{1}{|p{4.9cm}|}{\centering \textbf{Location(B)} 
									   \\ (Latitude, Longitude, Zipcode)
                                       } & 
\multicolumn{1}{|p{2.8cm}|}{\centering 21 \\11.0\%}  \\ \hline

\multicolumn{1}{|p{4.9cm}|}{\centering \textbf{App Generated Unique Identifiers(C)}
										\\ (Device Fingerprint ID, Install ID, Identity ID, Generated ID, UID (User ID), Attribution ID, Hardware ID, Placement ID)     
                                        } & 
\multicolumn{1}{|p{2.8cm}|}{\centering 19 \\10.0\%}  \\ \hline

\multicolumn{1}{|p{4.9cm}|}{\centering \textbf{All categories above (A+B+C)}} & 
\multicolumn{1}{|p{2.8cm}|}{\centering 70 \\36.7\%}  \\ \hline

\hline
\end{tabular}
\end{adjustbox}
\caption{Summary of our findings from Request key analysis. \textmd{Analyzing the \totalSignatures signatures for \totalApps apps from our crowdsourced signature database we found $~$31\% of apps leak at least one of the PII types.}}
\label{tab:AppKeyLibraryAnalysis}
\end{table}

\GS{New: }\textbf{Taxonomy of Keys containing PII:} Since our signatures are created using key-value pairs from the HTTP requests, it is possible to look for known PII (such as IMEI and Android ID) and identify all associated keys across different apps. For example, some of the keys associated with Android ID are \texttt{Android-ID,  X-CRASHLYTICS-ANDROID-ID, DeviceID}. Analyzing the \totalSignatures signatures for \totalApps apps from the signature server database, we discovered that $~$31\% of apps leak at least one of the PII types (see Table \ref{tab:AppKeyLibraryAnalysis}). Since many apps use the same libraries, we can potentially improve \PP's coverage for apps we have not seen before if they use keys known to be associated with PII leaks. While there are some challenges here, for example reliably identifying libraries based on names of keys, success here could help mitigate the cold start problem for apps not yet in our database.\GS{End}


\subsection{Battery Consumption}
%Since, we are doing the PII detection on the device itself, it is bound to negatively affect the battery life of the device. Apart from the display screen, the major battery drain in Smartphones is caused by the WiFi \cite{PathakEProfBattery}.

In Section \ref{sec:impl}, we discussed the various optimizations we did to reduce the energy overhead of running \PP, which we measured to be 30\% higher without our techniques. To quantify impact on battery life, we installed the top 20 apps from ``Free in Android Apps'' on our test devices. For the first test, we launched these apps (in the background) and then put the device in standby mode (screen off). In the second test, we used the MonkeyRunner script to open each of these 20 apps one by one, and interacted with them by performing 100 clicks on the screen (screen is on in this case). To measure overhead, we calculate the time it took for the battery to go from from 100\% to 85\% with and without \PP enabled. Note, to mimic typical user settings, we enabled the WiFi radio, LocationServices, etc on the test device and ran each test thrice to report data. Table \ref{tab:table_batterylife} presents the energy overhead results. Our data shows that for standby, \PP reduces battery lifetime by 9.7\% - 11.0\%, while for the active use case the overhead can be up to 14.2\%. 
% Since the dominant state of most users' devices is in standby, we believe the overheads are acceptable although we are investigating techniques to reduce this overhead further.


% \SC{included \KK{To make the comparison meaningful both tests should have the screen on at the same brightness. screen takes up a lot of battery}}

% SC{included} \KK{Are the screens on during the test? How about WiFi etc?}

%\KK{\GS{It should be Overhead}unclear what this means. 30\% faster than without \PP?}
%\SC{included. Running tests now}\YA{This is for the non-interactive case? i.e. you launch some apps and then let them run in the background with the screen turned off correct? We would need to make the case why we don't evaluate during regular usage (maybe because its hard to replicate?).} 

 
\subsection{User Survey} 

\label{sec:user_survey}

% Additionally, 7 users downloaded \PP from Play Store and took the same survey without explicit requirement.

% The participants were asked to keep \PP running for as long as possible and use their devices as they normally do. After 3 days, the option to take the Survey was available and the participants were asked to take the Survey from the app.

%\JH{Is there a Google doc somewhere of the survey results? Will be easier if I can see that too. Need to describe the questions and the scale. Need enough details for others to replicate.}

%CBDR (for anonymity).
% So our users are probably more tech savvy than the average mobile user.

We conducted an in-app user survey to measure perceived usability and performance overhead of \PP. The survey was delivered after 3 days of using \PP. All questions were on a 5-point Likert scale. 
For battery consumption, 85\% (23/27) of survey participants said that they ``Noticed no perceptible change''. 67\% (18/27) said the same about network performance. Although there is a performance overhead of using \PP, 54\% (14/26) of participants agreed that the performance overhead was worth the privacy improvement while 31\% (8/26) were neutral. Overall, 59\% (16/27) of users were able to use \PP without noticing any perceptible change to apps. 

\begin{table}
\small
  \begin{tabular}{|l|l|l|l|l|}
    \hline
	
    \multicolumn{1}{|p{1.8cm}|}{\centering Scenario} &
    \multicolumn{2}{|c|}{Samsung S7 Edge} & \multicolumn{2}{|c|}{Nexus 5x}  \\ \cline{2-5}
    
     	 & StandBy & \multicolumn{1}{|p{1.2cm}|} {\centering Monkey Runner} & 
         StandBy & \multicolumn{1}{|p{1.2cm}|} {\centering Monkey Runner} \\
    \hline
    \multicolumn{1}{|p{1.8cm}|}{\centering Without PrivacyProxy } & 
    	\multicolumn{1}{|p{1.1cm}|} {\centering 463 min} &
    	\multicolumn{1}{|p{1.1cm}|} {\centering 52 min} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 650 min} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 70 min} \\
    \hline
    \multicolumn{1}{|p{1.8cm}|}{\centering With PrivacyProxy } & 
    	\multicolumn{1}{|p{1.1cm}|} {\centering 416 min 	\\10.2\%} &
    	\multicolumn{1}{|p{1.1cm}|} {\centering 46 min 		\\11.5\%} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 594 min 	\\8.6\%} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 61 min 		\\12.8\%} \\
    \hline
    \multicolumn{1}{|p{1.8cm}|}{\centering With PrivacyProxy and Filtering } & 	 		
    	\multicolumn{1}{|p{1.1cm}|} {\centering 412 min 	\\11.0\%} &
    	\multicolumn{1}{|p{1.1cm}|} {\centering 45 min 		\\13.4\%} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 587 min 	\\9.7\%} &
        \multicolumn{1}{|p{1.1cm}|} {\centering 60 min 		\\14.2\%} \\
    \hline
  \end{tabular}
  	\caption{Battery Overhead Evaluation. \textmd{The percentage depicts the reduction in battery life, which varied from 12.8\% to 14.2\% in our 2 test devices.}}
	\label{tab:table_batterylife}
\end{table}

==> old_files/implementation.tex <==
\section{Implementation}
\label{sec: Implementation}

\JH{Implementation section should be relatively short. Should keep all of the design rationale in the earlier section. This part should just be about what software used, libraries, lines of code, etc. Everything should be in earlier sections.}

In this section we describe our implementation of PrivacyProxy, highlighting how we support our design goals mentioned in Section \ref{sec: System Design}. We first describe the features of Android and APIs which we used. Next we describe the PrivacyProxy app itself that users install on their devices. Finally, we describe the back end infrastructure and our crowdsourced signature detection system. Lastly, we also discuss optimization design decisions we made to improve the runtime performance, reduce power consumption still maintaining coverage.

\subsection{Android Platform Features}
PrivacyProxy is built on top of PrivacyGuard \cite{PrivacyGuard}. Since the VPN server runs on the IP layer, we need to use raw sockets to transmit IP datagrams directly. Android does not allow using raw sockets with root access.

\td{Wording feels off here, the VPN server doesn't run on the IP layer per se, does it process data at the IP layer? Also, who is it transmitting IP datagrams to? Writing is ambiguous above.}

To analyze the network flows leaving the device we used Android's VPNService API. This was added in API level 14. As mentioned in Section \ref{sec: System Design}, apps like Facebook and WhatsApp had implemented certificate pinning. To reduce the network latency we white listed these apps statically on the PrivacyProxy app. Before API 21, the packet was captured and bypassed in the processing state. This added network latency. API 21 added the methods to disallow apps from the VPN Service itself \cite{WhitelistApps}, reducing the network latency.

API 23 added the DozeMode optimization\cite{DozeMode}. We optimized the app for DozeMode to improve the battery life of the device. This is discussed in Section \ref{sec: Evaluation}. 

%included \SC{Add stuff about Location PII detection edge case.}

\JH{What is DozeMode? Why is it important? That is, why are you telling readers about it?}

\begin{figure*}
\centering
\begin{tabular}{cccc}
\tcbox[sharp corners,top=-3pt,left=-3pt,right=-3pt,bottom=-3pt]{{\includegraphics[width = 1.5in]{W1}}} &
\tcbox[sharp corners,top=-3pt,left=-3pt,right=-3pt,bottom=-3pt]{{\includegraphics[width = 1.5in]{W2}}} &
\tcbox[sharp corners,top=-3pt,left=-3pt,right=-3pt,bottom=-3pt]{{\includegraphics[width = 1.5in]{W3}}} &
\tcbox[sharp corners,top=-3pt,left=-3pt,right=-3pt,bottom=-3pt]{{\includegraphics[width = 1.5in]{W4}}} \\
\end{tabular}
\caption{\textmd{Screenshots of the PrivacyProxy app, from left to right: (a) Home screen showing summary information, (b) a list of monitored apps along with summary information for each app, (c) drill-down information for a specific app, showing key-value pairs that have been sent off the device, (d) Settings Screen for purpose-based filtering}}
\label{fig:PrivacyProxyScreenShots}
\end{figure*}

\subsection{PrivacyProxy Android App}
We designed the \textit{PrivacyProxy} app which runs on an Android device running Android API 15 to API 24. Figure \ref{fig:system_architecture} illustrates the different PrivacyProxy modules at a high level, as well as their interconnection and how they interact with the backend server. The app has been tested on devices running Android 4.3, Android 5.0, Android 5.1, Android 6.0 and Android 7.0 in the lab. We ported PrivacyGuard to Android Studio 2.2.2 and made 3324 lines of modification. Our Android code to design the PrivacyProxy app contains 30,000 lines of code. 

%SC{included}\td{Below, this is the third or fourth mention of using PrivacyGuard for the VPN. Need to tighten up the text to be less repetitive}

\subsection{Signature Server}
The Signature Server is responsible for handling private signature uploads and public signature downloads. When a user uploads their private signature, the server combines the private signature with the public signature and stores the public signature in a database for later retrieval by all other users. The properties of Count-min Sketch makes combining signatures trivial. In addition, each Count-min Sketch in a signature can be updated independently, so we don't have to worry about users having slightly different signatures with the same SID. The Signature Server is implemented as a simple HTTPS server implemented in 1009 lines of Go. In addition, there are 351 lines of scripts used to analyze the results, written in Go. We use the Let's Encrypt SSL Certificate for HTTPS and MySQL as our database.
% \td{stores it in a database... what does the "it" refer to in this part of the text?} \SC{it is the private signature} 

To minimize the amount of storage needed and to minimize users' bandwidth, we use Google's Protobuf library to efficiently serialize all signatures for transmission and storage. Note that in our current implementation, we use 64 bit integers to implement Count-min Sketch, so each key only takes up $5 \times 55 \times 8 = 2200$ bytes in a signature regardless of the number of values.

% \td{Is it each key or each key-value?}
% \KK{Each key takes up 2200 bytes regardless of the number of values}

To protect users' privacy, we do not record the IP address of each upload or create any identifier to associate a user with the signatures that they have uploaded. To avoid the problem of one user uploading multiple copies of the same private signature, we programmed the app to enforce the policy that every private signature may only be uploaded once. In addition, we only allow the upload of signatures that include at least 10 observations in order to ensure that we get quality signatures while limiting users to only upload them once. \YA{does this mean if a key0value is send by a device once we won't send that signature?} Currently, to protect against a malicious actor from uploading fake signatures in hopes to skew the probability estimates, we randomly discard a fraction of uploaded signatures (note that this feature is not enabled in our lab tests) \td{Should say what the current fraction is}. \YA{to prevent sybil attacks, we could use better techniques rather than just randomly throwing them away?} The exact probability for discarding uploads directly affects the rate at which our signatures grow, and we defer the task of deciding its value to future work. \YA{this seems to be punting.} Another possible way to mitigate the problem of malicious uploads is to compare the frequency estimates from the uploaded signature to those from the signature stored in the database. If the frequencies are substantially different, we can weigh the uploaded requests more lightly when combining signatures or hold off on the combining step until we see more signatures with the same SID to do the comparison again. \td{I'm having a hard time understanding which of these measures have been implemented. Is the random discard implemented? What about frequency comparison? It might also be easier to move this to a separate section about security too.} \YA{I agree, this section is vague and unclear what's been done in reality.} \GS{Both of these are not implemented, but this is to suggest possible solutions and that we have considered there is a posibility of Sybil attack. We can mention the PMP way. I think. Its more structured.}

\textbf{Scalability} is part of our solution by design. After a signature has accumulated information from several uploaded signatures, combining it with a new signature does not dramatically change the estimates generated by the signature. Therefore, we have very relaxed atomicity and consistency requirements for our Signature Server. \YA{why are we concerned about ACID properties? This only becomes an issue if we have distributed Signature servers no?} 

This means that we can deploy a DNS-like hierarchical architecture to scale up our Signature Server, where SIDs are URLs and signatures are the DNS records. We can \YA{we can, but do we?} split up the SID namespace into different zones while maintaining a set of core name servers that can be reached via IP anycast. Each Signature Server handles user uploads by aggregating a new signature locally and doing batch updates to their peers. The server can also aggressively cache signatures and name server records since we are not concerned about staleness. Furthermore, if we add a field to each Count-min Sketch that stores the number of times the key-value pair represented by that Count-min Sketch has been classified as PII, then we can allow the server to service a signature request by picking Count-min Sketches that are most likely to contain PII and sending them to the client. The same technique applies for signature uploads. This allows us to limit the amount of signature data that must be transferred to avoid taking up too much of the user's bandwidth. As shown in the next section, most requests contain less than 10 pieces of PII, so this method is quite feasible. \YA{you have to be clear on what *can* be done, and what we *have* implemented. Else its all comes across as vaporware/ideas only.}

\td{The above discussion is good, but is making it hard to know what has and has not been implemented. It's better to move the above to a discussion section about scalability, rather than here about implementation.}
\KK{I agree, this is good for the discussion section since none of it is actually implemented it.}

\subsection{Confidence levels}
\td{\GS{Added by me}Very Important: Discussion about confidence levels , "Highly Identifiable" $(Private_prob - Public_prob) = >80\%$ , "Moderately Identifiable 80-20\%", "Low Identifiable below 20\%" }

\subsection{Performance Optimization}
%Comment Included: \YA{ All the performance optimizations can go under implementation, since these are all systems issues that we encountered while implementation right?}

%Saksham
\SC{Adding stuff about Edge cases}\\
While designing the system and testing in our lab setting we discovered several challenges. First, in our crowdsourced system, location PII was dependent upon the geographical spread of our user base. If a majority of the users were at a single location, then Location would be marked as an Application Constant instead of PII. Note that this issue would be solved by a big enough user base. We implemented an alternate approach where potential PII would be compared against the last known location of the device. Second, the time stamps were being updated and transmitted constantly by apps and libraries like Yelp, SpeedTest, and Google Analytics. We infer that this is to prevent caching \cite{GoogleAnalyticsTrackingCode}. To prevent \PP from marking this value as PII we compared the time stamp being sent with the current time. If the time stamp is within an hour of the current time, then we do not mark it as PII. This would also ensure that the install time UNIX time stamps which is used to track users would be detected as PII. Third, many apps like Facebook, WhattsApp and Google Play Store had enabled certificate pinning which did not allow us to monitor or filter their traffic. The apps gave a time out and did not work with PrivacyProxy turned on. To maintain the usability of the app, we statically whitelisted these apps from the VPN Service. Furthermore, if an app didn't load correctly on 3 tries we infer that it has enabled certificate pinning and we whitelist it dynamically. Finally, battery life and performance of the device were a major concern while building a usable product. To improve the performance, we implemented a Fast Path approach, where if an app version was not leaking any PII after 500 requests we put it on Fastpath and do not monitor the traffic for that app version. We discuss more about Battery Life optimizations in the Section \ref{sec:Evaluation}.
%\SC{Not talking about battery life here. We discuss it in the Evaluation Section.}
% included \SC{Should the other edge cases like location and time stamp pii detection be added here as well?}

\textbf{Statistical Fast Path:} As additional optimization steps, we temporarily stop monitoring (Fast Path) applications based on the statistics from their previous requests. The key idea is that if on a user's device an application makes many internet requests and after a certain number of requests we did not detect any potential PII leaks, it is safe to ignore that application's requests for performance reasons. Although, as soon as the app tries to contact a new host and path combination which it has not in previous requests we start monitoring (Slow Path) the app requests. The rationale behind this is that the request structure remains same for same path and host and since we don't find any leaks in previous request, it is less likely that future request to same host and path would have PII. This gives us significant improvement in phone performance. We discuss the performance in evaluation section. 

\textbf{Server Side Whitelisting:} Along similar lines we implemented Server side whitelist. If there are more than 5 users for an app and on aggregate users have seen enough request with no PII detected its very much possible that the app doesn't leak PII. We calculate these numbers from our telemetry service we get aggregate information (App Name, No of Requests, No of Potential PII flagged by \PP). When a new user installs \PP app, these whitelisted apps are fetched from our RESTful service and added to bypass VPN if the user has the app installed. This provides a key advantage for new users that they will not waste processing power on monitoring these apps which most likely don't leak PII.

Screenshots of PrivacyProxy app, from left to right: (a) The Home Screen, where Clicking on the Button would turn the VPN Service on and off, (b) 



==> old_files/ppoverview.tex <==
\section{PrivacyProxy Overview}
\label{sec:PrivacyProxyOverview}
%As discussed in previous sections, the problem of apps leaking users private data to third-parties (Advertisers, Analytics companies, application performance monitors, or crash reporters.) is widely known. The state-of-the-art approaches either require users to be tech savvy or thrust a 3-rd party to protect data giving access to the 3rd party or have limitation to detect only pre-configured or well known PII. To address the limitations of current approaches and address the design goals discussed in Section \ref{sec: System Design}, we have built 

PrivacyProxy uses on-device network analysis and crowdsourcing to detect likely PII leaks from Android devices. As noted earlier, we focus on one specific form of PII, namely unique identifiers. We also propose a novel signature based detection approach which allows us to identify likely PII without any a priori knowledge about the structure of those identifiers. PrivacyProxy also  mitigates information leakage by allowing the user to mark detected values as PII and filter them from network requests before they leave the device without disrupting the app's behavior.

\subsection{System Architecture}
Figure \ref{fig:system_architecture} shows an overview of PrivacyProxy's system architecture. PrivacyProxy runs as a VPNService to intercept the network traffic from all apps. Since the VPN operates at the IP layer, the app extracts the payload from each IP packet to obtain the transport layer packet and use that information to open a socket to communicate with the \textbf{\textit{LocalServer}}. Thus, from the perspective of the apps, the \textit{LocalServer} is the destination host that they are talking to. Note that \PP is not a real VPN client. Instead, it just poses itself as one to intercept network traffic leaving the phone. 

\KK{{I think we want to mention that our system is based on PrivacyGuard here (instead of only in the implementation section) because some terminology such as LocalServer is from them. Also, we make references to it in the following paragraphs. }}

\td{What's the LocalServer? The description above isn't quite crisp. Also, suggest talking about SSL and certificates below too.}

\SC{Should we talk about SSL and certificates in the implementation section instead?}

\td{I don't understand the below, why does it combine data into an HTTP request? Isn't it already an HTTP request?}
\SC{The Local Server receives the data in form of Network packets. So the request has to be reformed. Made this distinction clear.}

After intercepting network data, the LocalServer's job is to 1) perform PII analysis and 2) forward the data to the real Internet destination. We refer interested readers to \cite{PrivacyGuard} for details on how forwarding is done. For every new connection to the LocalServer, a \textbf{\textit{RequestParser}} combines every piece of raw packet data on the connection into HTTP requests. These HTTP requests are then turned into signatures by the \textbf{\textit{SignatureGenerator}} and saved in the Signature Database. We chose to operate on HTTP requests because they are very common among Android apps \cite{A_First_Look_at_Traffic_on_Smartphones} (our tests show that at least 70\% of the apps analyzed contained HTTP traffic) and are highly structured, though we propose a possible alternative design in Section \ref{sec:Conclusions} that applies our approach to raw byte streams.

% we create a thread to run the \textbf{\textit{RequestParser}}, Add in implementation part later

\subsection{Extracting Key-Value Pairs} 
For each HTTP request that we encounter, we try to extract key-value pairs that contain application-specific data from the request. Figure \ref{fig:HTTPRequest} shows an example request and the key-value pairs that would be extracted. We extract all the arguments in the request URI and ignore all common headers such as ``Accept-Encoding" and ``Content-Type" since they are unlikely to contain PII. For uncommon headers such as ``X-Secret-Location-Header", we treat it as a key-value pair, but we try to parse the value associated with the header as JSON, XML, or URL since the value may be formatted. If none of the 3 methods work, then we just treat the value as plain-text. Similarly, for the message body, we use hints such as the ``Content-Type" header to determine how to parse it. If we cannot determine the type of the body, then we try all 3 formats and if none of them work, we simply treat the body as one big value and assign a fixed key for it. This is not robust against users who use proprietary encoding or serialization libraries such as Google's Protobuf where we do not know the schema to decode the messages. However, in our tests, only 0.5\% of the HTTP requests contain special encoding that we cannot parse. 

\SC{We can probably remove the below part if space is a constraint}\\
In order to avoid conflicting keys, we generate each key according to its position in the request. All keys in the request URI are prepended with ``U", while those in the header and the body are prepended with ``H" and ``B", respectively. In addition, a key in a nested structure will have all the keys in its parent structures prepended to it.

\td{Double check for above, is the proper term "request URI" or "URL path"?}
\SC{URIs identify and URLs locate and identify. So should be "request URI"}\\
\JH{For above, might allude to limitations, e.g. data that isn't well-structured, like blobs}
\SC{Included}\\

% Yuvraj: removed since moved to a new file. 
% \begin{figure*}
% \centering
% \begin{adjustbox}{center, width=(\columnwidth-10pt) * 2}
% \begin{tabular}{ccc}
%  {
%    \includegraphics[height=4cm,width=6cm]{HTTPRequest}
%    \label{fig:HTTPRequest}
%  } &
%  {
%    \includegraphics[height=4cm,width=6cm]{SignatureStructure}
%    \label{fig:signature_structure}
%  } &
%  { \includegraphics[height=4cm,width=6cm]{SingleCount-Min}
%    \label{fig:signature_structure}
%  } \\
% \end{tabular}
% \end{adjustbox}
% \caption{\textmd{Signature Generation Process flow : (a) Our Request Parser looks for key-value pairs in app HTTP requests, looking at query parameters in URL paths, HTTP headers, and the payload. Extracted Key-Value Pairs are highlighted. (b) Signature structure on our server for the HTTP Request in Figure 2. A signature identifies the app used, destination, URL Path, and method, as well as Count-min sketch for all keys. c) Count-min sketch for key: Device\_ID in HTTP Request: Count-min sketch is a probabilistic and compact data structure that can count the frequency of different values seen for each key.}}
% \end{figure*}
% \KK{The image of the HTTP request has an extra line above Referer}

\td{1. Show the whole system overview diagram. The current diagram does not include the part of how the VPN works, that should be included and new components should be added too like : 1. Filter 2. Data Predictor 3. Policy Enforcer }
\GS{Updated System Architecture Images}

\td{Below, does SID stand for something? Is it signature ID? Also, does the signature refer to what is sent to our servers, stored by our servers, or both?}
\SC{Yes, it is Signature id. Signature refers to both what is sent to our servers and what is stored in our servers.}\\

\subsection{Signature Generation}
Signatures form the basis of our crowdsourced PII detection algorithm. Each signature is identified by the tuple (package name, app version, method, host, path), which we refer to as an \textit{SID} or Signature ID. This allows us to associate HTTP requests with their corresponding signatures. For example, if the HTTP request in Figure \ref{fig:signature_structure} was sent from the app io.privacyproxy.app, it would have the corresponding SID of (io.privacyproxy.app, 1.0, GET, www.privacyproxy.io, /api/v1). Note that the use of SID allows us to associate a signature with the same requests sent by the same app from different users' devices. The use of app and host to separate requests into different signatures is important for PII detection, which is explained in the next section.

We generate a signature from the key-value pairs that are extracted from all the HTTP requests with the same SID. For each key in the requests, the signature stores a Count-min Sketch \cite{CountMinSketch} that records the frequencies of all the different values that are associated with a given key, as illustrated in Figure \ref{fig:signature_structure}. 

\JH{how do we know the app name? Is PrivacyProxy using a process monitor? Or is it looking at some network table? Also, is this the signature on our server, or the signature that is sent? I'm guessing on our server, but need to clarify.}
\GS{The app name comes from the signature while signature generation we know where the traffic is coming from}\\
\JH{Lastly, suggest showing an example of different values and counts in the figure.}
\SC{This part is a bit ambiguous could you explain?}\\

\textbf{Count-min Sketch} is like a 2-dimensional Bloom filter that can estimate the frequency of some event. Concretely, each Count-min Sketch is a collection of \(r\) integer arrays of length \(n\) (every element initialized to 0) and \(r\) hash functions. It supports 2 operations: \(increment(v)\) and \(count(v)\). The \(increment\) function takes in a value \(v\) and for each array $\alpha_i ( 1 \leq i \leq r )$, it increments the integer at $\alpha_i[hash_i(v)]$ by one. The count function returns an estimate on the frequency of the value v by returning $min_{1\leq i \leq r}(\alpha_i[hash_i(v)])$ . Note that the Count-min Sketch is extremely space efficient since it only requires $r \times n$ integers. Given any value, it will either return the correct frequency or an overestimate of the frequency (but never an underestimate). In addition, it does not reveal the actual values that were inserted. Multiple Count-min Sketches can also be trivially combined by doing a element-wise sum over each array. In our implementation, we use SHA-256 as the hash function and we generate \(r\) different hash functions by appending fixed random strings to the value \(v\). Furthermore, for each Count-min Sketch, we also maintain a counter \(m\) which keeps track of the number of times the increment function was called, regardless of the value used. We chose $r = \lceil \ln \frac{1}{0.01}\rceil = 5 $ and $n = \lceil \frac{e}{0.05}\rceil = 55 $, which theoretically ensures that if the true frequency of \(v\) is $f_v$, then $P[count(v) \leq f_v + 0.05m] \geq 0.99$.

\td{I don't quite get the equation above, should it be two leq's instead of a leq and geq? Also, what's the intuition behind the equation above? What should readers get from it?}

There are two types of signatures: private and public. \textbf{Private Signatures} are generated by each user.
\textbf{Public Signatures} are generated by combining private signatures that are uploaded to the Signature Server by different users. Since the signatures themselves don't reveal any information other than the SID, there are minimal privacy concerns. We note that while we can get the IP address of the uploader, a user can easily use Tor or other services to hide their IP Address. We acknowledge that the combining step in public signature generation presents a malicious actor an opportunity for a possible Sybil attack. We discuss the mitigation strategies in section \ref{sec:security}.

% included \td{For limitations, may want to add that an attacker could potentially poison our signature database, we don't have a good defense against that yet.} 

\td{How Private Signatures are created and merged which keeps the anonymity of the user. And also how Private Probability is calculated from the Private Signature for a key-value pair}
\td{Discuss about how the Public Signatures are created by Periodically uploading private signatures and \textbf{Merging} it with public signature from the crowdsourced DB. Anonymous for user/ Not actual values transmitted}
\td{Discuss about the signature key, how they provide a unique way of grouping PII and also how this can provide different \textbf{Granularity} for PII Control eg. Purpose based, App Based, Blocking for a Host (Hence Library based) }
\td{Discuss how the Count-min Sketch works.\\
Also why Count-min sketch rather than directly storing the value, Ans: Count-min doesn't need to store the actual value and hence Anonymous and saves space, but still gives a good approximation of the frequency of a value}


\begin{table*}
\centering
\begin{adjustbox}{center, width=(\columnwidth-10pt) * 2}
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
%Header
Experiment & Parameter & 
\multicolumn{1}{|p{1.9cm}|}{\centering MAC ID Device ID Email ID (A)} &
\multicolumn{1}{|p{1.9cm}|}{\centering IP Address Location Phone Number(B)} &
\multicolumn{1}{|p{1.9cm}|}{\centering App Specific IDs / Token / License (C)} &
\multicolumn{1}{|p{2.2cm}|}{\centering True Positive (A $\cup$ B $\cup$ C)} &
\multicolumn{1}{|p{2.2cm}|}{\centering False Positive $\neg$(A $\cup$ B $\cup$ C)} &
\multicolumn{1}{|p{2.2cm}|}{\centering Precision} 
\\ \hline
%Rows
\multicolumn{1}{|p{2.cm}|}{\centering Controlled Lab Experiment} & 
\multicolumn{1}{|p{2.5cm}|}{\centering Top 100 apps + 2 Nexus 5, Android 5.1.1} & 
90 & 60 & 20 & 200 & 12 & .94\\ 
\hline

\multicolumn{1}{|p{2cm}|}{\centering User Study} &
\multicolumn{1}{|p{2.5cm}|}{\centering Top 100 apps + 25 random users} & 
90 & 60 & 20 & 300 & 34 & .89\\ 
\hline

\multicolumn{1}{|p{2cm}|}{\centering Tester App} &
\multicolumn{1}{|p{2.5cm}|}{\centering All possible PII + over HTTP and HTTPS} &
90 & 60 & 15 & 5 & 0 & 1.0\\ 
\hline

\end{tabular}
\end{adjustbox}
\caption{Summary of PII leaks detected from our experiment. \textmd{We present all well known PII which were detected and app specific PII which were detected by \textit{PrivacyProxy}. The values which \textit{PrivacyProxy} predicted as PII and apparently doesn't belong to any of the 3 categories are an over approximation False Positives. Note that \textit{PrivacyProxy} is novel in identifying any previously unknown PII which is a limitation of all current approaches which is grouped under category C}}
\label{table:precision}
\end{table*}

\subsection{Detecting Likely PII}
\label{sec:detection_mechanishm}
Our detection algorithm is based on a straightforward premise. Given a key-value pair extracted from a request, how many users have seen a similar value? If the answer is very few or none, then we infer that the value is likely PII since it is associated with a specific user more often than with other users. For example, a unique user ID should always be present in a user's request but is different across all users' requests. On the other hand, if a request contains the package name of the app, then it should be the same in all users' requests. \KK{I don't think this belongs here: During our experiments we discovered that many applications tend to send current time in terms of the number of milliseconds since the Unix Epoch, which can be classified as PII since it is unlikely that two users use the same application at the exact same millisecond. Although, we also discovered that some of the potential fingerprinting attacks where apps transmit the app install time as milliseconds as fingerprinting ids. We discuss this in detail in section \ref{sec: Evaluation}.} A corner case for our detection approach is Location in cases where multiple users are using \textit{PrivacyProxy} at the same place. In this case our algorithm may not detect location as a leak since the same coordinates are in requests from different users. We will discuss the approaches we used to handle these cases in section \ref{sec: Implementation}. 

% included \td{Should mention exception cases upfront, which we'll discuss later. For example, timestamps, location data, etc.}
\td{Although as our Crowd DB grows large enough with many users with same app, these timestamps and locations would be detected properly}

Let $S_{private}$ and $S_{public}$ represent the private and public signature for a given request, respectively. We'll use the notation $F (S, k, v)$ to denote the estimated frequency for the value $v$ associated with key $k$ as reported by signature $S$. Likewise, we'll use the notation $C(S, k)$ to denote the number of values (not-necessarily unique) that have been inserted into signature $S$ for key $k$. \YA{confused about the Frequency F and the Count C here}. For each key-value pair $(k, v)$ extracted from the request, let $P_{private}(k, v)$ be the estimated probability of seeing the pair in the user's own requests and let $P_{public}(k, v)$ be the estimated probability of seeing the pair across different users' requests. We can then calculate $$P_{private}(k, v) = \frac{F(S_{private},k,v)}{C(S_{private},k)}$$ 
Likewise for $P_{public}(k, v)$. \\
%\KK{fixed} \YA{the 'key=value' pairs are what are used right? So, should the formula not be 'k-v' rather than just 'v'?}

Let's consider the PII analysis for a given key-value pair $(k,v)$. For brevity, we'll use $P_{private}$ to refer to $P_{private}(k, v)$ and $P_{public}$ to refer to $P_{public}(k, v)$. We'll let $T$ be a threshold
value between 0 and 1 that is "sufficiently large" and can be tuned. Using these information, we can classify $(k, v)$ into 3 categories:
\setdefaultleftmargin{0pt}{}{}{}{}{}

\td{Are the equality signs going in the right direction?}

\begin{enumerate}
  \item \textbf{Application Constant} 
  $$P_{private} \geq T$$ 
  $$P_{private} \leq P_{public}$$ 
  
% SC{included} \YA{I'd put these in two separate lines and clarify that we need both to be true.}
\YA{we also need to say what T is, and what its value will typically be for each of these cases.} The values in this category are present in most requests for the user. However, they also appear frequently in the requests of other users.
%However, it is not particularly special when compared to requests from other users. 
We call values in this category as application constants since they are likely to be constant for all the requests with the same SID. A good example would be developer IDs that are used by ad libraries to identify the app that made the ad request in order to pay the developer. The ability to detect values in this category shows why we chose to include package name and host in the SID. We don't want to mix application constants from different apps together and risk diluting the probability of seeing those values, which might lead us to misclassify them as context-sensitive data.
  \item \textbf{Context-Sensitive Data} $$P_{private} < T$$ Values in this category are not very common among the requests from the user. Thus, they are unlikely to be a PII or application constants. There are 2 possible explanations for values in this category. The first is that the value may be generated on the fly by the app for specific purposes. Examples include timestamps, random numbers generated by libraries such as Google Analytics to prevent caching \cite{GoogleAnalyticsTrackingCode}, and application specific checksums. The second possibility is that the value is associated with the user's actions. Examples include the number of minutes the screen is on or the user's precise GPS location if the user frequently changes location.In general, it is hard to determine whether values in this category are privacy sensitive or not. Our current solution is to defer the decision to the user and let them decide whether the information looks sensitive or not.
  \item \textbf{Personally Identifiable Information(PII)}$$P_{private} \geq T$$ 
  $$P_{private} > P_{public}$$ 
%\YA{I'd put these in two separate lines and clarify that we need both to be true.} \SC{included}
  
  For values to be classified as PII, they need to appear in a large fraction of a single user's requests while appearing infrequently in other user's requests.
  %Values in this category are almost certainly PII since they appear in a large fraction of the user's requests but are not as common among other user's requests.
\end{enumerate}

The selection of $T$ is fairly flexible as long as it is ``sufficiently large'' to prevent context-sensitive values from being misclassified as PII or application constants. \YA{this is vague, and putting quotes does not make it better. We need to say that this is a parameter that can be tuned to reduce false positives ..and say how we choose this T for our tests} Currently, we set $T = \frac{3}{4}$ based on empirical results from our tests.\td{Once I have graph for $T$ relation it would be good addition here for selection of $T$} Since we ask the user to identify whether a piece of context-sensitive data is privacy sensitive or not, we can include a $T$ field in every Count-min Sketch and incorporate the user's feedback to adjust it. Another possibility is to expose $T$ to the user as a control of how much "autonomy" the proxy has. The higher the value of $T$ is, the more reliant the proxy is on user input to classify context-sensitive data. \td{Not sure, it should, the lower the T more values are identified and we rely more on user to tell us what is PII right?}

Note that the properties of Count-min Sketch means that we'll never underestimate $P_{private}$
and $P_{public}$. Along with theoretical guarantees on the bounds of $count(v)$, our PII detection algorithm is quite conservative in determining whether a given value is a PII or not.\\ \YA{meaning that we err towards false positives?}
\SC{Yes. Bloom filters can err towards false positives}

The \textbf{crowdsourcing} aspect of our PII detection algorithm relies on public signatures from different users. The early adopters of \PP will not gain much since our coverage would be very low in terms of the number of apps that we have signatures for, though we note that we only need 2 users using the same app in order to provide basic PII detection for that app. As more users use \PP, not only will our signature coverage improve, but classification is going to become more accurate as well since each public signature will include more counts from different users to allow us to better estimate the distribution of different values. We can also crowdsource the decision of whether a key contains context-sensitive data by suggesting default values for $T$ based on the values used by different users.

==> old_files/systemdesign.tex <==
\section{System Design}
\label{sec: System Design}

\td{
1. Crowdsourced: Each user takes a small hit on performance and makes the solution efficient for others\\
2. Should be capable of Detecting and Filtering the Private Information\\
3. Identify the purpose of the PII leaks and provide fine-grained control to user\\
4. Maintain Usability of mobile device (JND)\\
}

\subsection{Research Goals}
We want to design a solution that can automatically detect and mitigate PII leaks from an Android device, subject to the following criteria: 
\begin{itemize}
\item \textbf{No OS/Device modification} We want users to be able to install and interact with the app without having to root or modify their devices. We chose this criteria so as to maximize the potential number of people who could use our app.

%\item \textbf{Crowdsourced PII Detection} Instead of using heuristics or machine learning techniques, we want to reliably determine whether a network flow contains PII via crowdsourcing. We will expand on this in section \ref{sec:detection_mechanishm}.

\item \textbf{Robustly detect unknown PII} By \textit{unknown}, we are referring to identifiers that are generated by individual apps or libraries. We should be able to detect these identifiers without prior knowledge about their value, type, or structure.

\item \textbf{Filter out specific PII} We want users to be able to filter out identifiers by removing them before they gets sent to a third-party.

\item \textbf{Usable} PrivacyProxy should work with little user intervention, and have minimal impact on battery life and app runtime performance. 

\item \textbf{Scalable} We want PrivacyProxy to scale well in terms of number of users and apps that can be covered. Ideally, the more users that use PrivacyProxy, the better it is in pinpointing identifiers.

\end{itemize}

\td{TODO: Discuss about the design goals. The things we are trying to balance out. \\
1. Performance (Detection, Mitigation) \\
2. Coverage (Of apps and leaks) \\
% Included 3. Phone Performance(Network Latency/Battery Life/ \\
4. Usability/Annoyance/Uninstall/Understand ability
5. Scalability/ Widespread adoption 
6. Robustness

old text: suggest moving this to implementation, this isn't really a goal: \textbf{App and library specific} The current permission based control is not adequate as the user has to decide to either use an app (functionality) or renounce privacy. We want to associate PII with the specific app or library that leaked it in order to enforce PII filtering at a per-app or per-library granularity.

}

\subsection{Threat Model}

We define our adversary model as Opportunistic adversary\\
Data comes at no additional cost for them (developer, 3-rd party library developer)\\
The solution strategies we propose:\\
1. Warn the user/ User awareness\\
2. Mitigation technique/Countering threat with preventive PET (Filtering)\\

\td{ We can define Opportunistic Threat model, the app developer's might not be particularly malicious but 1. Risk reward and can act in a stealthy manner for if there is some reward and chances of being caught or held accountable is very meager}

\begin{comment}
\subsection{Challenges}
\td{TODO: Discuss about the factors which we are trying to balance out, from the above list of goals and how they counter each other to create a pull-push scenario and how we balance them to find the best possible path}
\td{Not sure we really need this section on Challenges, can discuss the tradeoffs in the next section when describing the design of PrivacyProxy- JIH}
\GS{Since we are discussing this in section 5.5 Performance Optimisation. Commenting this section.}
\end{comment}

\begin{figure}
\centering
\includegraphics[width=8cm]{SystemArchitecture}
\caption{PrivacyProxy system architecture. PrivacyProxy runs as a VPN on an end-user's Android smartphone. The Request Parser parses an app's HTTP requests, looking for key-value pairs in the HTTP headers, the URL, and  JSON or XML payloads. The Signature Generator creates signatures based on the app name, app version, URL, and key-value pairs. New signatures that have not been previously uploaded are sent to our Signature Server. PrivacyProxy also gets counts of signatures it has seen, allowing the PII Detector it to infer likely PII. The Request Filter uses an end-user's rules to decide whether to scrub out PII before it leaves the phone.}
\label{fig:system_architecture}
\end{figure}
